The Tarantula -- Revealed by X-rays (T-ReX)

The Tarantula Nebula (30 Doradus) is the most important star-forming complex in the Local Group, offering a microscope on starburst astrophysics. At its heart lies the exceptionally rich young stellar cluster R136, containing the most massive stars known. Stellar winds and supernovae have carved 30 Dor into an amazing display of arcs, pillars, and bubbles. We present first results and advanced data processing products from the 2-Ms Chandra X-ray Visionary Project, "The Tarantula - Revealed by X-rays" (T-ReX). The 3615 point sources in the T-ReX catalog include massive stars, compact objects, binaries, bright pre-main-sequence stars and compact young stellar (sub)clusters in 30 Dor. After removing point sources and excluding the exceptionally bright supernova remnant N157B (30 Dor B), the global diffuse X-ray maps reveal hot plasma structures resolved at 1-10 pc scales, with an absorption-corrected total-band (0.5-7 keV) X-ray luminosity of $2.110\times 10^{37}$ erg s$^{-1}$. Spatially-resolved spectral modeling provides evidence for emission lines enhanced by charge-exchange processes at the interfaces. We identify a candidate for the oldest X-ray pulsar detected to date in 30 Dor, PSR J0538-6902, inside a newly-resolved arctuate X-ray wind nebula, the Manta Ray. The long time baseline of T-ReX monitored dozens of massive stars, several showing periodic variability tied to binary orbital periods, and captured strong flares from at least three low-mass Galactic foreground stars.

==> VFTS_and_Doran_matches.tex <==
%\documentclass[preprint,11pt,trackchanges]{aastex63}
%
%\usepackage{grffile}  %grffile allows .'s in filenames
%\usepackage{url}
%\newcommand{\tablenotetextbox}[3]{\vspace{\baselineskip}\hspace{-0.6in}#1\hspace{1ex}\parbox[t]{#2}{#3}}
%\newcommand{\tnm}[1]{\tablenotemark{#1}}
%
%\begin{document}
% Reduce the space between table columns.
\setlength{\tabcolsep}{1mm}

\begin{longrotatetable}
\startlongtable
%\begin{deluxetable}{@{}lrrrrllllllchp{0.7in}p{1.4in}lp{1.0in}@{}}
\begin{deluxetable}{@{}lrrrrllllllcchhhp{1.0in}@{}}
%\movetableright=-1in
\movetabledown=0.5in
\tablewidth{10in}
\tabletypesize{\tiny}
\tablecolumns{14}
\tablecaption{Candidate and Known Massive Stars With Counterpart in 1910 X-ray Sources Defined in Table~\ref{tbl:OIR_catalogs} \label{tbl:massive_matches}}       
\tablehead{
 \multicolumn{4}{c}{X-ray Source} &
 \multicolumn{4}{c}{VFTS/Doran ID, Adopted Coordinates\tablenotemark{a}} &
 \colhead{} &
 \multicolumn{3}{c}{Other Counterpart Names} &
%\multicolumn{2}{c}{Spectral Type}
\\[-5pt]
 \multicolumn{4}{c}{\hrulefill} &
 \multicolumn{4}{c}{\hrulefill} &
 \colhead{} &
% \colhead{} &
 \multicolumn{3}{c}{\hrulefill} &
%\multicolumn{2}{c}{\hrulefill}
\\[-8pt]
 \colhead{Label} &     
 \colhead{NetCt} & %\colhead{NetCounts\_t} &
 \colhead{PhotonFlux\_t} & % \colhead{Flux} & 
 \colhead{$E_{med}$} & % \colhead{MedianEnergy\_t} &
 \colhead{ID} &
 \colhead{RA} &
 \colhead{DEC} & 
 \colhead{Src} &
 \colhead{Sep.\tablenotemark{b}} & 
 \colhead{Gaia} &
 \colhead{VMC} &
 \colhead{HTTP\tablenotemark{c}} &
 \colhead{See also\tablenotemark{d}} &
 \nocolhead{Other} &  % Identifiers reported by Evans11 or SIMBAD.
 \nocolhead{Type} &
 \nocolhead{Ref.} &
 \colhead{Notes}
\\[-12pt]
 \colhead{} &
 \colhead{ct} &
 \colhead{ph~cm$^{-2}$~s$^{-1}$} &
 \colhead{keV} &
 \colhead{} &
 \colhead{} &
 \colhead{} &
 \colhead{} &
 \colhead{\arcsec} &
 \colhead{\#46576} &
 \colhead{\#55834} &
 \colhead{} &
 \colhead{} &
 \colhead{} 
}
%\colnumbers                     \nodata             
\startdata
\multicolumn{12}{l}{\bf\footnotesize Declared Counterparts in VFTS Catalog}\\
  c893     &  73& 2.63E-7& 1.2&  16        & 05:37:08.881 & -69:07:20.37 &G  & 0.61 &  90620070706432 & 9005257 &053708.880-690720.33 &C22           &  & O2III-If* & Walborn & \\ % good match
  c3084    &  43& 1.04E-7& 1.2& 186        & 05:37:52.033 & -69:04:39.79 &G  & 0.41 &  80621362544384 & 8981182 &053752.028-690439.90 &C22           &  &  &  & \\ % good match
  p1\_441  & 181& 4.36E-7& 1.1& 217        & 05:37:59.488 & -69:09:01.66 &G  & 0.29 &  79964217679104 & 9020340 &053759.487-690901.73 &C22           & ST92 1-98 & O4V((fc)):+O5V((fc)):, SB2 & Walborn & \\ % good match
  c3981    &  22& 5.46E-8& 1.4& 259        & 05:38:12.027 & -69:06:34.16 &G  & 0.42 &  80518305213184 & 8998543 &053812.019-690634.21 &C22           &  & O6Iaf, SB1s & Walborn & \\ % good match
  p1\_480  & 169& 4.18E-7& 1.4& 267        & 05:38:13.966 & -69:07:47.72 &G  & 0.07 &  79934189673088 & 9012687 &053813.961-690747.85 &C22           &  & O3III-I(n)f*, SB1vs & Walborn & \\ % good match
  p1\_553  &  59& 1.37E-7& 0.9& 333        & 05:38:23.714 & -69:05:03.55 &G  & 0.16 &  80479615199616 & 8984799 &053823.706-690503.57 &C22           & R133, P93-0042  & O8II-III((f)), SBvs & Walborn & \\ % good match
  c4876    &  68& 1.76E-7& 1.1& 352        & 05:38:28.461 & -69:11:19.12 &G  & 0.36 &  78216202797440 & 9041783 &053828.463-691119.12 &C22           &  & O4.5V(n)((fc)):z:+O5.5V(n)((fc)):z:, SB2 & Walborn & \\ % good match
  c5200    &  12& 3.56E-8& 1.0& 385        & 05:38:32.310 & -69:05:23.85 &G  & 0.23 &  86286410990464 & 9019931 &053832.293-690523.85 &C22           & P93-0288, S99-084 & O4-5V((n))((fc)), SBs & Walborn & \\ % good match
  p1\_610 &22077& 4.93E-5& 3.2& 399        & 05:38:33.413 & -69:11:59.02 &G  & 0.13 &  77456003693440 & 9048274 &053833.417-691159.00 &C22 C15       & See C15. & O9IIIn & Walborn & X-ray binary\\ %good match 
  p1\_611  & 140& 3.74E-7& 4.7& 402        & 05:38:33.624 & -69:04:50.50 &G  & 0.03 &  86290742293888 & 9019904 &053833.615-690450.47 &C22 T19       & R135, S99-012, Brey 80, BAT99-095. See T19. & WN7h & Evans & \\ % good match
  c5349    & 146& 3.96E-7& 1.4& 404        & 05:38:33.834 & -69:09:57.06 &G  & 0.06 &  79831110499840 & 9028504 &053833.835-690957.04 &C22           &  & O3.5V(n)((fc)), SB1l & Walborn & \\ % good match
  c5374    &  20& 4.77E-8& 1.1& 406        & 05:38:33.980 & -69:04:21.22 &G  & 0.63 &  86325102023552 & 8978318 &053833.969-690421.17 &C22           & Mk 55, P93-0370 & O6Vnn & Walborn & marginal match: Gpos well outside ACIS error box (Aerrbx);  Asrc on HTTP streak\\ % Evans11 says "Some cross-contamination".
  cc4181   &   7& 2.12E-8& 0.8& 410        & 05:38:34.610 & -69:06:05.86 &V  & 0.18 &                 & 9020004 &053834.587-690605.87 &C22           & P93-0409, S99-288 & O7-8V,VM3 & Walborn & \\ % good match
  cc4200   &   7& 2.39E-8& 1.4& 411        & 05:38:34.787 & -69:05:00.55 &G  & 0.25 &  86286459752064 &         &053834.779-690500.53 &C22           & S99-409 &  &  & \\ % good match
  c5572    &  17& 8.69E-8& 1.1& \tnm{e}416 & 05:38:35.576 & -69:06:06.68 &G  & 0.12 &  80415225904640 & 9020071 &053835.570-690606.65 &C22           & S99-093 &  &  &  \\ % good match %Doran \& VFTS may be duplicates;
  cc4294   &   2& 8.60E-9& 2.5& 417        & 05:38:35.664 & -69:06:17.48 &G  & 0.24 &  80415225921920 &         &053835.657-690617.45 &C22           & S99-204 & B2Ib & McEvoy & \\ % good match
  c5633    &  11& 3.64E-8& 0.9& 420        & 05:38:35.947 & -69:06:09.25 &G  & 0.03 &  80415225947008 & 9020008 &053835.941-690609.23 &C22           & Mk 54, P93-0488, S99-016 & B0.5Ia,Nwk, SB1? & McEvoy & \\ % good match
  p1\_637  &  66& 1.69E-7& 1.7& 427        & 05:38:36.411 & -69:06:57.53 &G  & 0.06 &  80380866211200 & 9020049 &053836.406-690657.48 &C22 T19       & Mk 53, S99-051, Brey 81, BAT99-096. See T19. & WN8(h) & Evans & \\ % good match
  p1\_663  & 215& 6.88E-7& 1.5& 445        & 05:38:38.033 & -69:05:43.34 &G  & 0.04 &  86290742451072 & 9019965 &053838.026-690543.30 &C22           & P93-0621, S99-097 & O3-4V:((fc)):+O4-7V:((fc)):, SB2 & Walborn & \\ % good match
  c5987    &  27& 8.53E-8& 1.2& 450        & 05:38:38.483 & -69:06:22.01 &G  & 0.19 &  79654981423744 & 9020076 &053838.476-690621.96 &C22           & Mk 50, P93-0643, S99-034 & O9.7III:+O7::, SB2 & Walborn & \\ % good match
  p1\_672  &  29& 1.03E-7& 1.3& 455        & 05:38:38.765 & -69:06:13.27 &G  & 0.25 &  79659312977536 & 9020016 &053838.759-690613.22 &C22           & P93-0661, S99-108 & O5:V:n, SB1l & Walborn & \\ % good match
  c6030    &  50& 1.61E-7& 1.5& 457        & 05:38:38.845 & -69:06:49.54 &G  & 0.13 &  79624951968640 & 9020045 &053838.838-690649.49 &C22 T19       & Mk 51, P93-0666, S99-050, BAT99-097. See T19. & O3.5If*/WN7 & CW11 & \\ % good match
  cc4601   &  15& 4.44E-8& 1.4& 460        & 05:38:38.994 & -69:06:58.94 &G  & 0.28 &  79624951969536 & 9000920 &053838.987-690658.89 &C22           & P93-0674, S99-278 & O7.5V+O7.5V & Walborn & \\ % good match
  c6094    &  13& 4.89E-8& 2.1& 465        & 05:38:39.275 & -69:06:39.01 &G  & 0.49 &  79659311706752 & 9020041 &053839.269-690638.96 &C22           & P93-0700, S99-365 & O5:Vn & Walborn & marginal match: Gpos well outside Aerrbx;  Asrc on faint HTTP light\\
  p1\_682  &  66& 1.94E-7& 1.2& \tnm{f}468 & 05:38:39.374 & -69:06:06.54 &G  & 0.06 &  79659312983808 & 9020006 &053839.369-690606.49 &C22           & Mk 36, P93-0706, S99-086 &  &  & \\ % good match % Doran \& VFTS may be duplicates (email 2015 Sept 1)
  p1\_698  &7988& 1.69E-5& 1.6& 482        & 05:38:40.221 & -69:05:59.91 &G  & 0.03 &  79659312960256 &         &053840.214-690559.86 &C22 T19       & Brey 78, Mk 39, P93-0767, S99-014. See T19. & O2.5If*/WN6 & CW11 & \\ % good match
  c6370    &  34& 1.39E-7& 3.4&1001        & 05:38:40.546 & -69:05:57.24 &G  & 0.1  &  85534828221824 &         &053840.539-690557.18 &C22 T19       & R134, S99-013. See T19. & WN6(h) & CD98 & \\ % good match
  cc4769   &  41& 9.01E-8& 1.8&1003        & 05:38:40.773 & -69:06:03.49 &G  & 0.18 &  79659312996608 &         &053840.766-690603.44 &              & S99-283 &  &  & \\ % good match
  p1\_722  &  93& 3.45E-7& 1.3& 500        & 05:38:41.218 & -69:02:58.35 &G  & 0.02 &  86084583863296 & 8968085 &053841.212-690258.34 &C22           &  & O6.5IV((fc))+O6.5V((fc)), SB2 & Walborn & \\ % good match
  c6701    &  61& 1.32E-7& 1.1&1014        & 05:38:41.509 & -69:06:00.97 &G  & 0.1  &  85534828236416 &         &053841.507-690600.92 &C22           & S99-056 & O2-4.5+mid/lateO & HB12 & \\ % good match
  p1\_749  & 113& 3.68E-7& 1.1& 506        & 05:38:41.556 & -69:05:19.49 &G  & 0.05 &  85534828092032 & 9019926 &053841.545-690519.43 &C22           & Mk 25, P93-0871, S99-019,  & ON2V((n))((f*)), SB1s & Walborn & \\ % good match
  p1\_752 &54076& 1.46E-4& 1.5& 507        & 05:38:41.601 & -69:05:13.45 &G  & 0.05 &  85569167442432 &         &053841.601-690513.43 &C22 T19       & Brey 87, R140N [Mk], R140a [M87], S99-006, BAT99-101  +  102. See T19. & WC4(+WN6+O) & Evans &  ACIS pile-up \\ %good match; R140a
  p1\_754  & 396& 1.51E-6& 1.7& 509        & 05:38:41.625 & -69:05:15.18 &G  & 0.03 &  85569188005248 &         &053841.613-690515.17 &C22 T19       & Brey 87, R140S [Mk], R140b [M87], S99-008, BAT99-103. See T19. & WN5h(h)+O(+earlyO) & Evans & \\ %good match; R140b
  p1\_760  &  71& 1.75E-7& 1.2& 512        & 05:38:41.741 & -69:06:25.08 &G  & 0.01 &  79655028521472 &         &053841.734-690625.01 &C22           & P93-0885, S99-068 & O2V-III((f*)), SB1l & Walborn & \\ % good match
  p1\_786  & 194& 4.99E-7& 1.5&1017        & 05:38:41.870 & -69:06:14.49 &G  & 0.03 &  79659312965632 &         &053841.862-690614.41 &C22           & S99-088 & O2If*/WN5 & CW11 & \\ %good match; useful figure to demonstrate crowded extraction
  p1\_795  & 157& 3.54E-7& 1.2&1019        & 05:38:42.009 & -69:06:07.63 &G  & 0.04 &  79659292338176 &         &053842.004-690607.56 &C22           & S99-070 & O3III(f*)+O8 & MH98 & \\ % good match
  c6973    &  38& 1.50E-7& 1.3&1021        & 05:38:42.079 & -69:06:14.37 &G  & 0.15 &  79659312965248 &         &053842.072-690614.32 &C22           & S99-025 & O4If* & MH98 & \\ % good match
  c6974    & 161& 3.84E-7& 1.5& 522        & 05:38:42.088 & -69:05:45.54 &G  & 0.04 &  85534807590784 & 9019972 &053842.082-690545.47 &C22           & S99-134 &  &  & \\ % good match
  c7031    &  27& 6.85E-8& 1.9& 526        & 05:38:42.243 & -69:08:32.35 &G  & 0.23 &  79487513122048 & 9015834 &053842.238-690832.29 &C22           & P93-0925 & O8.5I((n))fp, SB1l & Walborn & \\ % good match
  p1\_830  &1680& 4.19E-6& 1.4& 527        & 05:38:42.359 & -69:04:58.19 &G  & 0.06 &  85564856502528 & 9019909 &053842.351-690458.19 &C22           & R139, Brey 86, P93-0952, S99-002 , BAT99-107 & O6.5Iafc+O6Iaf & T11 & \\ % good match
  c7131    &  90& 2.31E-7& 1.5&1022        & 05:38:42.403 & -69:06:15.14 &G  & 0.15 &  79659312957312 &         &053842.397-690615.08 &C22           & Mk 37, S99-028 & O4If* & MH98 & \\ % good match
  c7254    &  21& 6.66E-8& 1.2& 532        & 05:38:42.663 & -69:06:35.89 &G  & 0.09 &  79659311801600 & 8997593 &053842.657-690635.83 &C22           & P93-0974, S99-104 & O3V(n)((f*))z+OB, SB1l/SB2? & Walborn & \\ % good match
  p1\_893  &6955& 1.69E-5& 1.8&1025        & 05:38:42.903 & -69:06:04.96 &G  & 0.02 &  85534828237440 &         &\nodata              &C22 T19       & R136c; Blend of S99 027 \& 063. See T19. & WN5h & CD98 & \\ % good match
  c7410    &  69& 1.50E-7& 1.3&1026        & 05:38:43.060 & -69:06:11.26 &G  & 0.09 &  79659312979200 &         &\nodata              &C22           & Blend of S99 076 \& 191 & O2-4.5+mid/lateO & HB12 & ACIS aperture includes Doran725\_dM (distinct from VFTS src in HTTP image)\\ %good match; 
  p1\_911  & 204& 4.63E-7& 1.5& 542        & 05:38:43.097 & -69:05:46.89 &G  & 0.05 &  85530496766336 &         &053843.080-690546.86 &C22 T19       & Mk 30, P93-1018, S99-024, BAT99-113; also observed in Field A5 of the IFU data. See T19. & O2If*/WN5+lateO/earlyB & Evans & \\ % good match
  p1\_924  & 261& 5.70E-7& 1.5& 545        & 05:38:43.208 & -69:06:14.51 &G  & 0.07 &  79659312999296 &         &053843.202-690614.44 &C22 T19       & Mk 35, P93-1029, S99-023; also observed in Field A3 of the IFU data. See T19. & O2If*/WN5 & CW11 & \\ % good match
  p1\_937  &  39& 8.65E-8& 0.9&1028        & 05:38:43.268 & -69:06:16.58 &G  & 0.19 &  79659312998144 &         &053843.263-690616.51 &C22           & Mk 35S, S99-037 & O3.5-4.5 & HB12 & \\ % good match
  c7528    &  21& 5.00E-8& 1.4&1029        & 05:38:43.350 & -69:05:47.62 &G  & 0.38 &  85534807652224 &         &053843.343-690547.55 &C22           & S99-087 &  &  & marginal match: Gpos well outside Aerrbx\\
  c7552    &  26& 6.43E-8& 1.2&1030        & 05:38:43.423 & -69:05:42.08 &G  & 0.17 &  85534828273024 &         &\nodata              &C22           & S99-335 &  &  & \\ % good match
  p1\_955  & 116& 2.77E-7& 1.1&1031        & 05:38:43.688 & -69:05:47.93 &G  & 0.09 &  85534807650304 &         &053843.684-690547.89 &C22           & S99-039 & O3V & MH98 & \\ % good match
  c7859    &  27& 1.39E-7& 1.4& 562        & 05:38:44.413 & -69:05:36.25 &G  & 0.04 &  85530545537920 & 9019947 &053844.406-690536.22 &C22           & Mk 26, P93-1150, S99-032 &  &  & \\ % good match
  p1\_1021 &  24& 8.15E-8& 1.1& 564        & 05:38:44.559 & -69:05:12.42 &G  & 0.09 &  85564905241856 & 9020062 &053844.553-690512.35 &C22           & S99-253 & O6-8V((f)) & Walborn & \\ % good match
  c7907    &  48& 1.33E-7& 1.5& 566        & 05:38:44.569 & -69:04:51.25 &G  & 0.12 &  85569187906048 & 9019906 &053844.558-690451.19 &C22           & Mk 23, P93-1163, S99-042 & O3III(f*) & Walborn & \\ % good match
  cc5383   &  19& 9.77E-8& 1.5& 579        & 05:38:44.975 & -69:05:07.75 &G  & 0.09 &  85569187903104 &         &053844.969-690507.65 &C22           & In 'Knot 1' [WB87]; P93-1201, S99-171 & O9:((n)), SB?,VM2 & Walborn & \\ % good match
  c8052    &  22& 5.45E-8& 1.2& 585        & 05:38:45.272 & -69:05:46.61 &G  & 0.3  &  85534807640832 &         &053845.279-690546.53 &C22           & P93-1231, S99-031; also observed in Field A5 of the IFU data & O7V(n), SB1l,VM2 & Walborn & \\ % good match
  c8112    &  54& 1.43E-7& 1.3& 591        & 05:38:45.692 & -69:06:22.56 &G  & 0.04 &  79659311713024 &         &053845.687-690622.49 &C22           & Mk 12, P93-1257, S99-011 & B0.2Ia & McEvoy & \\ % good match
  c8160    &  64& 1.65E-7& 1.1& 599        & 05:38:46.183 & -69:06:17.47 &G  & 0.2  &  85534828283904 & 9020021 &053846.177-690617.39 &C22           & P93-1311, S99-040 & O3III(f*), SB1s & Walborn & \\ % good match
  p1\_1062 &  32& 8.67E-8& 1.4& 601        & 05:38:46.286 & -69:05:59.40 &G  & 0.13 &  85534828217856 & 9019999 &053846.280-690559.32 &C22           & Mk 14N, P93-1317, S99-091 & O5-6V((n))z & Walborn & \\ % good match
  c8180    &  22& 5.40E-8& 1.2& 603        & 05:38:46.539 & -69:04:28.04 &G  & 0.23 &  85672267222144 & 9019893 &053846.529-690427.99 &C22           & Mk 10, P93-1341 & O4III(fc), SB1l & Walborn & \\ % good match
  c8204    &  24& 6.38E-8& 1.1& 608        & 05:38:46.791 & -69:06:03.18 &G  & 0.24 &  85534828230528 & 9020002 &053846.785-690603.10 &C22           & Mk 14, P93-1350, S99-064 & O4III(f), SB1l & Walborn & \\ % good match
  p1\_1088 & 693& 1.74E-6& 1.4& 617        & 05:38:47.522 & -69:00:25.28 &G  & 0.23 &  87733851287040 & 8944472 &053847.533-690025.23 &C22 T19       & HDE 269926, R146, Sk-69 245, Brey 88, BAT99-117, P93-9033. See T19. & WN5ha & Evans & \\ % good match
  c8320    &  17& 6.79E-8& 1.8& 621        & 05:38:48.098 & -69:04:42.28 &G  & 0.18 &  85667984452864 & 9019899 &053848.089-690442.18 &C22           & In 'Knot 2' [WB87]; P93-1429 & O2V((f*))z,VM3 & Walborn & \\ % good match
  cc5800   &   6& 1.76E-8& 0.9& 640        & 05:38:49.665 & -69:08:54.84 &G  & 0.45 &  79418793663232 & 9019102 &053849.664-690854.73 &C22           & P93-1489 &  &  & \\ % good match
  c8591    &  24& 6.29E-8& 1.0& 648        & 05:38:50.407 & -69:05:38.26 &G  & 0.45 &  85500468549248 & 8989552 &053850.400-690538.17 &C22           & Mk 08, P93-1531, S99-058 & O5.5IV(f) & Walborn & marginal match: Gpos well outside Aerrbx, but nothing else closer\\
  p1\_1186 & 152& 4.02E-7& 1.4& 664        & 05:38:52.728 & -69:06:43.24 &G  & 0.02 &  85466108826624 & 9018610 &053852.724-690643.13 &C22           & Mk 04, P93-1607, S99-065 & O7II(f), SB? & Walborn & \\ % good match
  p1\_1234 & 302& 7.14E-7& 2.1& 682        & 05:38:55.527 & -69:04:26.80 &G  & 0.03 &  85637907503744 & 8979450 &053855.519-690426.72 &C22 T19       & P93-1732. See T19. & WN5h & Evans & \\ % good match
  p1\_1256 & 784& 1.87E-6& 2.0& 695        & 05:38:57.072 & -69:06:05.65 &G  & 0.06 &  85500468567040 & 9018590 &053857.072-690605.58 &C22 T19       & HDE 269928, R145, Sk-69 248, Brey 90, P93-1788, BAT99-119. See T19. & WN6h+? & Evans & \\ % good match
  p1\_1274 &   4& 1.05E-8& 3.3& 703        & 05:38:58.564 & -69:07:52.59 &G  & 0.63 &  79556232625408 & 9018687 &053858.561-690752.46 &C22           & P93-1828 & O7:V:+O8:V:, SB2 & Walborn & \\ % good match
  c10098   &  17& 4.01E-8& 1.3& 746        & 05:39:07.328 & -69:07:46.07 &G  & 0.63 &  79384433945344 & 9008310 &053907.327-690745.93 &C22           &  & O6Vnn & Walborn & VFTS src outside Aerrbx\\
  c10271   &  31& 7.36E-8& 1.2& 755        & 05:39:10.921 & -69:06:13.73 &G  & 0.25 &  85397389373184 & 8994892 &053910.913-690613.63 &C22           & P93-2041 & O3Vn((f*)) & Walborn & VFTS src just outside Aerrbx; \\ % good match
  c10289   &  99& 3.13E-7& 2.5& 758        & 05:39:11.324 & -69:02:01.56 &G  & 0.38 &  85977170493568 & 8960269 &\nodata              &C22 T19       & HD38344, R147, Sk-69 251, Brey 92, BAT99-122. See T19. & WN5(h) & Evans & VFTS src just outside Aerrbx; \\ % good match
  cc7769   &   5& 1.50E-8& 0.7& 768        & 05:39:16.235 & -69:01:20.38 &G  & 0.67 &  87493333392256 & 8958260 &\nodata              &C22           &  & O8Vn,NC & Walborn & \\ % good match
  cc7873   &   0& 1.79E-9& 4.2& 774        & 05:39:18.679 & -69:07:47.35 &G  & 1.03 &  85191230965760 & 9014727 &053918.676-690747.25 &C22           &  & O7.5IVp+O8.5:V:, SB2/SB3? & Walborn & \\ % good match
  p1\_1530 &  26& 6.68E-8& 0.9& 830        & 05:39:39.752 & -69:04:30.30 &G  & 0.35 &  82854768769024 & 9014580 &\nodata              &C22           & P93-2270 & O5-6V(n)((f)), SBl & Walborn & \\ % good match
% c5223 is "tentative" Pb_min=0.0018                                                               &          
% c5223    &  15& 0.9& 386        & 05:38:32.560 & -69:04:32.04 &V+ & 0.28 &                 &         &          & Mk 58(e), P93-0294 & O9IV(n), SB1l,VM2 & Walborn & \\ % good match
% c5334 is "tentative" Pb_min=0.0048                                                               &          
% c5334    &  10& 3.2& 400        & 05:38:33.543 & -69:05:21.75 &G  & 0.44 &  86290721633664 &         &          & P93-0348, S99-227 &  &  & HTTP \#471508 is closer to Asrc, but we have decided to keep the match to VFTS src\\
% cc4596 is "tentative" Pb_min=0.0025                                                              &          
% cc4596   &   9& 2.9& 459        & 05:38:38.961 & -69:03:12.17 &G  & 0.45 &  86462540979200 & 8976446 &          & P93-0684 &  &  & \\ % good match
% cc4785 is "tentative" Pb_min=0.0042                                                              &          
% cc4785   &  14& 1.1& 490        & 05:38:40.835 & -69:10:08.98 &G  & 1.2  &  79075196272128 & 9030179 &          &  &  &  & cc4785 (1.2\arcsec away), cc4765 (1.5\arcsec away) may have split light from VFTS source (Gpos).  No HTTP light on either ACIS src.\\
% cc4787 is "tentative" Pb_min=0.0058                                                              &          
% cc4787   &  11& 2.4&1005        & 05:38:40.969 & -69:06:08.45 &G  & 0.33 &  79659312963456 &         &          & S99-330 & O4V((f))+O6 & MH98 & pretty good match; HTTP \#408271 closer but much fainter\\
% cc4832 is "tentative" Pb_min=0.0015                                                              &          
% cc4832   &   6& 1.2& 501        & 05:38:41.245 & -69:04:14.29 &G  & 0.4  &  85667984679296 &         &          & P93-0849 & O9/B0V & Bosch & \\ % good match
% c8042 is "tentative" Pb_min=0.0017                                                               &          
% c8042    &   9& 1.5& 584        & 05:38:45.251 & -69:06:54.93 &G  & 0.56 &  79659290054144 & 9018750 &          & S99-443 &  &  & marginal match:  VFTS src $\sim$0.4\arcsec away (Gpos), well outside Aerrbx;  HTTP\#341438 matches Asrc\\
% cc5938 is "tentative" Pb_min=0.0033                                                              &          
% cc5938   &  14& 1.3& 652        & 05:38:51.048 & -69:06:20.49 &G  & 0.16 &  85461824464896 & 8996311 &          & Mk 05, P93-1552, S99-054 & B2Ip+O9III, SB2 & Walborn & \\ % good match
% cc6008 is "tentative" Pb_min=0.0059                                                              &          
% cc6008   &   9& 1.4& 660        & 05:38:51.819 & -69:05:46.94 &G  & 0.72 &  85496137040896 & 8990613 &          & P93-1586, S99-224 & O9.5Vnn & Walborn & marginal match:  VFTS src $\sim$0.7\arcsec away (Gpos), well outside Aerrbx; much fainter HTTP \#386140 matches Asrc\\
% cc6625 is "tentative" Pb_min=0.0054                                                              &          
% cc6625   &  12& 1.1& 706        & 05:38:58.774 & -69:05:23.98 &G  & 0.34 &  85599216261376 & 9019934 &          & P93-1838 & O6-7Vnnz & Walborn & \\ % good match
% cc6709 is "tentative" Pb_min=0.001027                                                            &          
% cc6709   &   0& 4.1& 713        & 05:38:59.900 & -69:08:14.78 &G  & 0.56 &  79350074201472 & 9018713 &          & P93-1868 &  &  & pretty good match; VFTS src just outside Aerrbx, but HTTP \#224553 \& \#224552 match Asrc\\
% cc7970 is "tentative" Pb_min=0.0052                                                              &          
% cc7970   &  11& 2.4& 779        & 05:39:21.541 & -69:03:18.45 &G  & 1.3  &  85912785446528 & 8969909 &          &  & B1II-Ib, SB1 & McEvoy & marginal match:  VFTS src $\sim$1.4\arcsec away (Gpos), not too far outside Aerrbx;  no HTTP light on Asrc\\
%
%
\\
\hline
\hline
\multicolumn{12}{l}{\bf\footnotesize Declared Counterparts in Doran13 Catalog}\\
  p1\_296 &1174 & 2.80E-6& 1.9& 185  & 05:37:49.039 & -69:05:08.21 &G   & 0.12 & 92338057418624 & 8986916 &053749.028-690508.33&C22 T19       & RMC 130. See T19.& WN/C+B1I & BAT99 & \\ % good match
  c4012   &  30 & 6.87E-8& 1.0& 273  & 05:38:13.162 & -69:05:36.41 &G   & 0.29 & 80655744058112 & 8991351 &053813.159-690536.51&              &                  &  &  & \\ % good match
  c5695   &  13 & 4.13E-8& 1.1& 398  & 05:38:36.243 & -69:06:08.46 &G   & 0.52 & 80415225947776 &         &053836.237-690608.42&C22           &                  &  &  & marginal match:  Doran src $\sim$0.4\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c5867   &  17 & 5.42E-8& 1.5& 415  & 05:38:37.438 & -69:05:50.34 &G   & 0.42 & 80415227189632 &         &053837.429-690550.30&              &                  &  &  & marginal match:  Doran src $\sim$0.4\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c5984   &  38 & 9.11E-8& 1.5& 427  & 05:38:38.454 & -69:04:17.98 &G   & 0.4  & 86423899131008 & 9019890 &053838.438-690417.94&C22           &                  & O8/9V & Bosch & \\ % good match
  c6062   &  65 & 1.92E-7& 2.8& 443  & 05:38:39.149 & -69:06:21.29 &G   & 0.1  & 79654981424640 & 9020032 &053839.143-690621.24&C22 T19       & Mk 49. See T19.  & WN6(h) & BAT99 & \\ % good match
  cc4651  &  41 & 9.88E-8& 1.7& 458  & 05:38:39.621 & -69:05:59.39 &G   & 0.16 & 79659312981760 & 9020000 &053839.614-690559.35&C22           &                  &  &  & \\ % good match
  c6164   &  10 & 4.51E-8& 1.2& 462  & 05:38:39.698 & -69:06:24.05 &G   & 0.32 & 79654981425664 & 9020034 &053839.692-690624.01&C22           &                  & O7III & Bosch & Doran462 (Gpos) between c6164,c6138 (just outside Aerrbx of c6164)\\
  c6170   &  22 & 7.69E-8& 1.4& 461  & 05:38:39.699 & -69:06:08.59 & D+ & 0.22 &                &         &053839.700-690608.63&C22           &                  &  &  & \\ % good match
  c6213   &  23 & 8.53E-8& 1.2& 472  & 05:38:39.853 & -69:06:09.55 &G   & 0.07 & 79659312983296 &         &053839.846-690609.50&C22           &                  &  &  & \\ % good match
  p1\_695 &  62 & 1.47E-7& 1.5& 475  & 05:38:40.150 & -69:05:51.31 &G   & 0.18 & 85530496759552 & 9019980 &053840.143-690551.26&C22           &                  & O3-6V & MH98 & \\ % good match
  p1\_711 & 124 & 3.49E-7& 1.5& 497  & 05:38:40.710 & -69:05:56.97 & D+ & 0.02 &                &         &053840.712-690556.99&              &                  &  &  & \\ % good match
  c6443   &  45 & 1.54E-7& 1.2& 502  & 05:38:40.805 & -69:05:25.15 &G   & 0.05 & 85534828067712 & 9019933 &053840.798-690525.10&C22           &                  & O5/6V & Bosch & \\ % good match
  p1\_718 &  45 & 1.23E-7& 1.3& 507  & 05:38:40.898 & -69:05:55.90 & D+ & 0.41 &                &         &053840.895-690555.93&C22           &                  &  &  & pretty good match; Doran src $\sim$0.4\arcsec away, well outside Aerrbx, but nothing else much closer\\
  c6472   &  22 & 7.76E-8& 1.2& 508  & 05:38:40.950 & -69:05:55.11 & D+ & 0.18 &                &         &053840.949-690555.14&C22           &                  &  &  & \\ % good match
  c6555   &  32 & 7.51E-8& 1.7& 521  & 05:38:41.150 & -69:05:49.45 &G   & 0.17 & 85534828224000 &         &053841.142-690549.40&              &                  &  &  & \\ % good match
  p1\_745 & 473 & 1.04E-6& 1.4& 539  & 05:38:41.488 & -69:05:56.89 & D+ & 0.08 &                &         &053841.490-690556.90&C22           &                  & O3V & MH98 & \\ % good match
  c6981   & 336 & 1.10E-6& 1.4& 576  & 05:38:42.079 & -69:06:02.22 & D+ & 0.08 &                &         &053842.081-690602.22&C22           &                  & O3V+O3-5V & MH98 & \\ % good match
  p1\_812 & 933 & 2.02E-6& 1.5& 580  & 05:38:42.112 & -69:05:55.33 &G   & 0.06 & 85534828234496 &         &053842.104-690555.29&C22           & Mk 42            & O2If* & CW11 & 3 other Doran srcs (573, 577, 587) in ACIS aperture, but this is definitely the best match\\ %good match; 
  cc4987  &  35 & 1.45E-7& 1.5& 604  & 05:38:42.259 & -69:06:00.46 & D+ & 0.13 &                &         &053842.258-690600.47&              &                  &  &  & \\ % good match
  cc4968  &  66 & 1.72E-7& 1.6& 612  & 05:38:42.308 & -69:06:04.94 & D+ & 0.2  &                &         &\nodata             &C22           &                  &  &  & in R136; dM position for Doran612; Doran600\_dM also in ACIS aperture\\
  c7109   &  36 & 1.67E-7& 2.6& 636  & 05:38:42.389 & -69:06:00.08 & D+ & 0.19 &                &         &053842.383-690600.09&              &                  &  &  & uncataloged HTTP source matches Asrc; Doran636 is just outside Aerrbx; in R136\\
  c7235   &   7 & 4.69E-8& 0.9& 677  & 05:38:42.623 & -69:05:36.79 &G   & 0.1  & 85534828074624 & 9020078 &053842.616-690536.74&C22           &                  & O6/7V((f)) & Bosch & \\ % good match
  p1\_867 & 522 & 1.61E-6& 1.4& 682  & 05:38:42.658 & -69:06:02.91 & D+ & 0.02 &                &         &\nodata             &C22           &                  & O3If* & MH98 & Doran682 uses dM position\\ %good match; 
  p1\_979 &2180 & 4.70E-6& 1.4& 765  & 05:38:44.129 & -69:05:56.71 &G   & 0.03 & 85534828260608 &         &053844.123-690556.63&C22           & Mk 33 Sa         & O3III(f*) & MH98 & \\ % good match
  p1\_995 &74445& 1.48E-4& 1.8& 770  & 05:38:44.256 & -69:06:06.00 &G   & 0.04 & 85534828257792 & 9020003 &053844.252-690605.93&C22 P18       & MK 34. See P18.  & WN5h & CD98 & ACIS pile-up \\ %good match; 
  p1\_1000&1865 & 4.09E-6& 1.5& 775  & 05:38:44.334 & -69:05:54.72 &G   & 0.02 & 85534828252672 &         &053844.329-690554.66&C22           & Mk 33 Na         & O3If* & MH98 & \\ % good match
  p1\_1033&  95 & 2.22E-7& 1.4& 800  & 05:38:44.958 & -69:05:54.18 &G   & 0.14 & 85534807639808 & 9020069 &053844.950-690554.11&C22           &                  & O3V & MH98 & \\ % good match
  c8022   &  16 & 5.78E-8& 2.2& 807  & 05:38:45.071 & -69:05:09.59 & D+ & 0.22 &                &         &053845.051-690509.73&              &                  &  &  & \\ % good match
  p1\_1035&  49 & 2.10E-7& 1.7& 810  & 05:38:45.148 & -69:05:08.46 &G   & 0.18 & 85564905253504 &         &053845.150-690508.34&C22           &                  & O3-6V & WB97 & \\ % good match
  p1\_1194&1233 & 2.90E-6& 1.8& 916  & 05:38:53.383 & -69:02:00.88 &G   & 0.1  & 86222022977920 & 8959289 &053853.363-690200.88&C22 T19       & RMC 144. See T19.& WN6h & BAT99 & \\ % good match
  cc8189  &  15 & 3.74E-8& 1.7& 1038 & 05:39:25.332 & -69:09:12.99 &G   & 1.09 & 76356437382656 & 9022508 &053925.334-690912.93&              &                  &  &  & \\ % good match
% c5887 is "tentative" Pb_min=0.0042                                                                           &
% c5887   &   7 & 1.3& 417  & 05:38:37.666 & -69:05:42.09 &G   & 0.27 & 86290742450048 & 9019960 &          &          & O3/5V & Bosch & \\ % good match
% cc5421 is "tentative" Pb_min=0.001042                                                                        &
% cc5421  &  16 & 1.3& 820  & 05:38:45.501 & -69:05:44.07 &G   & 0.52 & 85534807640576 & 9020081 &          &          &  &  & marginal match:  Doran src $\sim$0.3\arcsec away (Gpos), well outside Aerrbx; HTTP \#410263 matches Asrc\\
% c8137 is "tentative" Pb_min=0.0013                                                                           &
% c8137   &  17 & 1.0& 831  & 05:38:45.914 & -69:05:50.85 &G   & 0.28 & 85534807638656 &         &          &          &  &  & good match; HTTP\#403892 inside Aerrbx\\
% cc7272 is "tentative" Pb_min=0.0032                                                                          &
% cc7272  &   5 & 1.8& 990  & 05:39:07.428 & -69:04:20.35 &G   & 0.14 & 85809706217856 & 8982007 &          &          &  &  & \\ % good match
%
%
\\
\hline
\hline
\multicolumn{12}{l}{\bf\footnotesize ACIS blends inside R136 cluster}\\
  p1\_987 &   84 &1.96E-7&1.2&\tnm{g}V1034  &&&G  & 0.2 &&&                    &C22       &Mk 32, S99-021& O8III(f)  & MH98 & Both could contribute to ACIS light\\ %VFTS1034 0.2\arcsec away (Gpos); Doran772\_dM 0.3\arcsec away; 
          &      &       &   &    D772      &&&D+ & 0.3 &&&                    &          &              & 06V       & MH98 & \\
\hline
  p1\_866 &   62 &1.50E-7&1.4&     D685     &&&G  & 0.25&&&                    &C22       &              &\nodata    && Both could contribute to ACIS light\\ %Doran685 is 0.25\arcsec away (Gpos); Doran671\_dM is 0.5\arcsec away;
          &      &       &   &     D671     &&&D+ & 0.5 &&&                    &          &              &\nodata    && \\
\hline
  p1\_832 & 4452 &1.15E-5&1.5&     D633     &&&D+ &     &&&                    &C22 T19   &R136a1/a2/a4/a5/a7/a8. See T19.& WN5h      & CD98 & Mushroom aperture at ACIS aimpoint; hopelessly confused at R136 core\\ % Doran 633,630,642,638 
          &      &       &   &     D630     &&&D+ &     &&&                    &          &              & WN5h      & CD98 & \\
          &      &       &   &     D642     &&&D+ &     &&&                    &          &              & O2If*     & CW11 & \\
          &      &       &   &     D638     &&&D+ &     &&&                    &          &              & O3III(f*) & MH98 & \\                                 
\hline
  p1\_766 &   31 &9.70E-8&1.6&\tnm{h}V513   &&&G  & 0.2 &&&                    &C22       & S99-266      & O6-7II(f) &Walborn& Both could contribute to ACIS light\\ %VFTS513 0.2\arcsec away (Gpos); VFTS515 0.4\arcsec away (NOT Gpos);
          &      &       &   &       V515   &&&V+ & 0.4 &&&                    &          & S99-434      &\nodata    && \\
\hline
  cc4970  &  496 &2.39E-6&1.7&    D613      &&&D+ &     &&&                    &C22 T19   & R136a3/a6. See T19.    & WN5h      & CD98 & $\sim$8 Doran srcs in ACIS aperture\\ %Doran 613,621  in R136; 
          &      &       &   &    D621      &&&D+ &     &&&                    &          &              &\nodata    && \\
\hline
  c7182   &  258 &6.18E-7&1.4&    D657      &&&D+ &     &&&                    &C22       &              & O3V       & MH98 & Many Doran sources in ACIS aperture\\ % Doran 657,652,649,659; in R136  
          &      &       &   &    D652      &&&D+ &     &&&                    &          &              &\nodata    && \\
          &      &       &   &    D649      &&&D+ &     &&&                    &          &              &\nodata    && \\
          &      &       &   &    D659      &&&D+ &     &&&                    &          &              &\nodata    && \\
\hline
  c7157   &  345 &8.16E-7&1.3&    D648      &&&D+ &     &&&                    &C22       &              & O3V       & MH98 & Many Doran sources in ACIS aperture\\ %Doran 648,624; in R136  
          &      &       &   &    D624      &&&D+ &     &&&                    &          &              & O3V       & MH98 & \\
\hline
  c7018   &   45 &2.20E-7&1.5&    D589      &&&D+ &     &&&                    &C22       &              &\nodata    && Many Doran sources in ACIS aperture\\ %Doran 589,583; in R136 
          &      &       &   &    D583      &&&D+ &     &&&                    &          &              &\nodata    && 
\enddata
\tablecomments{
Reported properties of ACIS sources (NetCounts\_t, PhotonFlux\_t, MedianEnergy\_t from Table~\ref{xray_properties.tbl}) are derived by combining all observations.  In some cases the source detection is most significant in a single observation.
NetCounts suggests the quality of the extracted spectrum, but is unsuitable for photometry.  Apparent Photon Flux (NetCounts / MeanEffectiveArea / ExposureTimeNominal) is a rough scaling of NetCounts to account for source-to-source variations in exposure time, effective area, and aperture size \citep[][\S7.4]{Broos10}.
}
%
\tablenotetextbox{a}{8in}{
The coordinates published in the VFTS and Doran catalogs were not directly used to assess positional coincidence between X-ray sources and candidate/known massive stars.
When the star could be identified in the Gaia catalog (Src ``G''), Gaia coordinates (propagated to the mean epoch of the \Chandra\ data, Y2014.5) and uncertainties were adopted.
Otherwise, when the star could be identified in the VMC catalog (Src ``V''), VMC coordinates were adopted and uncertainties were estimated by the authors.
Otherwise, pubished VFTS coordinates (``V+ '') were corrected using a field distortion map derived using Gaia and uncertainties were estimated by the authors.
Otherwise, published Doran coordinates (``D+ '') were corrected using frame shifts derived using Gaia and uncertainties were estimated by the authors.\\
}
%\vspace*{3em}
\tablenotetextbox{b}{8in}{
Separation between ACIS source and star's Adopted Coordinates; median is 0.15 arcsec.
}
\tablenotetextbox{c}{8in}{
Source label in the HTTP catalog.  Due to space limitations, our corrected HTTP positions are not reported.
}
\tablenotetextbox{d}{8in}{
Modeling of the T-ReX spectrum is described by 
\citet[C22]{Crowther22},
\citet[T19]{Tehrani19},
\citet[P18]{Pollock18},
\citet[C15]{Clark15}.
}
%\tablenotetextbox{e}{8in}{
%We suspect that the identifiers VFTS416 and Doran390 refer to the same star.
%}
%\tablenotetextbox{f}{8in}{
%We suspect that the identifiers VFTS468 and Doran451 refer to the same star.
%}
%\tablenotetextbox{g}{8in}{
%We suspect that the identifiers VFTS1034 and Doran769 refer to the same star.
%}
%\tablenotetextbox{h}{8in}{
%We suspect that the identifiers VFTS513 and Doran558 refer to the same star.
%}
%\tablecomments{Spectral Type References: 
%(1) Evans et al. 2011; (2) Foellmi et al. (2003); (3) Crowther \& Smith (1997); (4) Smith et al. (1990); (5) Conti \& Massey (1989); (6) Crowther \& Dessart (1998); (7) Bartzakos et al. (2001); (8) Moffat et al. (1987); (9) Massey \& Hunter (1998); (10) Smith et al. (1996); (11) Schmutz \& Vacca (1991); (12) Crowther \& Hadfield (2006); (13) Walborn et al. (1999); (14) Torres-Dodgen \& Massey (1988); (15) de Koter et al. (1997), (16) Breysacher (1986); (17) De Marchi et al. (2011); (18) Schnurr et al. (2008).
%}
\end{deluxetable}
\end{longrotatetable}


%\end{document}





==> massive_matches.tex <==
\setlength{\tabcolsep}{1mm}

\begin{longrotatetable}
\startlongtable
%\begin{deluxetable}{@{}lrrrrllllllchp{0.7in}p{1.4in}lp{1.0in}@{}}
\begin{deluxetable}{@{}lrrrrllllllcchhhp{1.0in}@{}}
%\movetableright=-1in
\movetabledown=0.5in
\tablewidth{10in}
\tabletypesize{\tiny}
\tablecolumns{14}
\tablecaption{Candidate and Known Massive Stars with T-ReX Detections \label{tbl:massive_matches}}             
\tablehead{
 \multicolumn{4}{c}{X-ray Source} &
 \multicolumn{4}{c}{VFTS/Doran ID, Adopted Coordinates\tablenotemark{a}} &
 \colhead{} &
 \multicolumn{3}{c}{Other Counterpart Names} &
%\multicolumn{2}{c}{Spectral Type}
\\[-5pt]
 \multicolumn{4}{c}{\hrulefill} &
 \multicolumn{4}{c}{\hrulefill} &
 \colhead{} &
% \colhead{} &
 \multicolumn{3}{c}{\hrulefill} &
%\multicolumn{2}{c}{\hrulefill}
\\[-8pt]
 \colhead{Label} &     
 \colhead{NetCt} & %\colhead{NetCounts\_t} &
 \colhead{PhotonFlux\_t} & % \colhead{Flux} & 
 \colhead{$E_{med}$} & % \colhead{MedianEnergy\_t} &
 \colhead{ID} &
 \colhead{RA} &
 \colhead{DEC} & 
 \colhead{Src} &
 \colhead{Sep.\tablenotemark{b}} & 
 \colhead{Gaia} &
 \colhead{VMC} &
 \colhead{HTTP\tablenotemark{c}} &
 \colhead{See also\tablenotemark{d}} &
 \nocolhead{Other} &  % Identifiers reported by Evans11 or SIMBAD.
 \nocolhead{Type} &
 \nocolhead{Ref.} &
 \colhead{Notes}
\\[-12pt]
 \colhead{} &
 \colhead{ct} &
 \colhead{ph~cm$^{-2}$~s$^{-1}$} &
 \colhead{keV} &
 \colhead{} &
 \colhead{} &
 \colhead{} &
 \colhead{} &
 \colhead{\arcsec} &
 \colhead{\#46576} &
 \colhead{\#55834} &
 \colhead{} &
 \colhead{} &
 \colhead{} 
}
%\colnumbers                     \nodata             
\startdata
\multicolumn{12}{l}{\bf\footnotesize Declared Counterparts in VFTS Catalog}\\
  c893     &  73& 2.63E-7& 1.2&  16        & 05:37:08.881 & -69:07:20.37 &G  & 0.61 &  90620070706432 & 9005257 &053708.880-690720.33 &C22           &  & O2III-If* & Walborn & \\ % good match
  c3084    &  43& 1.04E-7& 1.2& 186        & 05:37:52.033 & -69:04:39.79 &G  & 0.41 &  80621362544384 & 8981182 &053752.028-690439.90 &C22           &  &  &  & \\ % good match
  p1\_441  & 181& 4.36E-7& 1.1& 217        & 05:37:59.488 & -69:09:01.66 &G  & 0.29 &  79964217679104 & 9020340 &053759.487-690901.73 &C22           & ST92 1-98 & O4V((fc)):+O5V((fc)):, SB2 & Walborn & \\ % good match
  c3981    &  22& 5.46E-8& 1.4& 259        & 05:38:12.027 & -69:06:34.16 &G  & 0.42 &  80518305213184 & 8998543 &053812.019-690634.21 &C22           &  & O6Iaf, SB1s & Walborn & \\ % good match
  p1\_480  & 169& 4.18E-7& 1.4& 267        & 05:38:13.966 & -69:07:47.72 &G  & 0.07 &  79934189673088 & 9012687 &053813.961-690747.85 &C22           &  & O3III-I(n)f*, SB1vs & Walborn & \\ % good match
  p1\_553  &  59& 1.37E-7& 0.9& 333        & 05:38:23.714 & -69:05:03.55 &G  & 0.16 &  80479615199616 & 8984799 &053823.706-690503.57 &C22           & R133, P93-0042  & O8II-III((f)), SBvs & Walborn & \\ % good match
  c4876    &  68& 1.76E-7& 1.1& 352        & 05:38:28.461 & -69:11:19.12 &G  & 0.36 &  78216202797440 & 9041783 &053828.463-691119.12 &C22           &  & O4.5V(n)((fc)):z:+O5.5V(n)((fc)):z:, SB2 & Walborn & \\ % good match
  c5200    &  12& 3.56E-8& 1.0& 385        & 05:38:32.310 & -69:05:23.85 &G  & 0.23 &  86286410990464 & 9019931 &053832.293-690523.85 &C22           & P93-0288, S99-084 & O4-5V((n))((fc)), SBs & Walborn & \\ % good match
  p1\_610 &22077& 4.93E-5& 3.2& 399        & 05:38:33.413 & -69:11:59.02 &G  & 0.13 &  77456003693440 & 9048274 &053833.417-691159.00 &C22 C15       & See C15. & O9IIIn & Walborn & X-ray binary\\ %good match 
  p1\_611  & 140& 3.74E-7& 4.7& 402        & 05:38:33.624 & -69:04:50.50 &G  & 0.03 &  86290742293888 & 9019904 &053833.615-690450.47 &C22 T19       & R135, S99-012, Brey 80, BAT99-095. See T19. & WN7h & Evans & \\ % good match
  c5349    & 146& 3.96E-7& 1.4& 404        & 05:38:33.834 & -69:09:57.06 &G  & 0.06 &  79831110499840 & 9028504 &053833.835-690957.04 &C22           &  & O3.5V(n)((fc)), SB1l & Walborn & \\ % good match
  c5374    &  20& 4.77E-8& 1.1& 406        & 05:38:33.980 & -69:04:21.22 &G  & 0.63 &  86325102023552 & 8978318 &053833.969-690421.17 &C22           & Mk 55, P93-0370 & O6Vnn & Walborn & marginal match: Gpos well outside ACIS error box (Aerrbx);  Asrc on HTTP streak\\ % Evans11 says "Some cross-contamination".
  cc4181   &   7& 2.12E-8& 0.8& 410        & 05:38:34.610 & -69:06:05.86 &V  & 0.18 &                 & 9020004 &053834.587-690605.87 &C22           & P93-0409, S99-288 & O7-8V,VM3 & Walborn & \\ % good match
  cc4200   &   7& 2.39E-8& 1.4& 411        & 05:38:34.787 & -69:05:00.55 &G  & 0.25 &  86286459752064 &         &053834.779-690500.53 &C22           & S99-409 &  &  & \\ % good match
  c5572    &  17& 8.69E-8& 1.1& \tnm{e}416 & 05:38:35.576 & -69:06:06.68 &G  & 0.12 &  80415225904640 & 9020071 &053835.570-690606.65 &C22           & S99-093 &  &  &  \\ % good match %Doran \& VFTS may be duplicates;
  cc4294   &   2& 8.60E-9& 2.5& 417        & 05:38:35.664 & -69:06:17.48 &G  & 0.24 &  80415225921920 &         &053835.657-690617.45 &C22           & S99-204 & B2Ib & McEvoy & \\ % good match
  c5633    &  11& 3.64E-8& 0.9& 420        & 05:38:35.947 & -69:06:09.25 &G  & 0.03 &  80415225947008 & 9020008 &053835.941-690609.23 &C22           & Mk 54, P93-0488, S99-016 & B0.5Ia,Nwk, SB1? & McEvoy & \\ % good match
  p1\_637  &  66& 1.69E-7& 1.7& 427        & 05:38:36.411 & -69:06:57.53 &G  & 0.06 &  80380866211200 & 9020049 &053836.406-690657.48 &C22 T19       & Mk 53, S99-051, Brey 81, BAT99-096. See T19. & WN8(h) & Evans & \\ % good match
  p1\_663  & 215& 6.88E-7& 1.5& 445        & 05:38:38.033 & -69:05:43.34 &G  & 0.04 &  86290742451072 & 9019965 &053838.026-690543.30 &C22           & P93-0621, S99-097 & O3-4V:((fc)):+O4-7V:((fc)):, SB2 & Walborn & \\ % good match
  c5987    &  27& 8.53E-8& 1.2& 450        & 05:38:38.483 & -69:06:22.01 &G  & 0.19 &  79654981423744 & 9020076 &053838.476-690621.96 &C22           & Mk 50, P93-0643, S99-034 & O9.7III:+O7::, SB2 & Walborn & \\ % good match
  p1\_672  &  29& 1.03E-7& 1.3& 455        & 05:38:38.765 & -69:06:13.27 &G  & 0.25 &  79659312977536 & 9020016 &053838.759-690613.22 &C22           & P93-0661, S99-108 & O5:V:n, SB1l & Walborn & \\ % good match
  c6030    &  50& 1.61E-7& 1.5& 457        & 05:38:38.845 & -69:06:49.54 &G  & 0.13 &  79624951968640 & 9020045 &053838.838-690649.49 &C22 T19       & Mk 51, P93-0666, S99-050, BAT99-097. See T19. & O3.5If*/WN7 & CW11 & \\ % good match
  cc4601   &  15& 4.44E-8& 1.4& 460        & 05:38:38.994 & -69:06:58.94 &G  & 0.28 &  79624951969536 & 9000920 &053838.987-690658.89 &C22           & P93-0674, S99-278 & O7.5V+O7.5V & Walborn & \\ % good match
  c6094    &  13& 4.89E-8& 2.1& 465        & 05:38:39.275 & -69:06:39.01 &G  & 0.49 &  79659311706752 & 9020041 &053839.269-690638.96 &C22           & P93-0700, S99-365 & O5:Vn & Walborn & marginal match: Gpos well outside Aerrbx;  Asrc on faint HTTP light\\
  p1\_682  &  66& 1.94E-7& 1.2& \tnm{f}468 & 05:38:39.374 & -69:06:06.54 &G  & 0.06 &  79659312983808 & 9020006 &053839.369-690606.49 &C22           & Mk 36, P93-0706, S99-086 &  &  & \\ % good match % Doran \& VFTS may be duplicates (email 2015 Sept 1)
  p1\_698  &7988& 1.69E-5& 1.6& 482        & 05:38:40.221 & -69:05:59.91 &G  & 0.03 &  79659312960256 &         &053840.214-690559.86 &C22 T19       & Brey 78, Mk 39, P93-0767, S99-014. See T19. & O2.5If*/WN6 & CW11 & \\ % good match
  c6370    &  34& 1.39E-7& 3.4&1001        & 05:38:40.546 & -69:05:57.24 &G  & 0.1  &  85534828221824 &         &053840.539-690557.18 &C22 T19       & R134, S99-013. See T19. & WN6(h) & CD98 & \\ % good match
  cc4769   &  41& 9.01E-8& 1.8&1003        & 05:38:40.773 & -69:06:03.49 &G  & 0.18 &  79659312996608 &         &053840.766-690603.44 &              & S99-283 &  &  & \\ % good match
  p1\_722  &  93& 3.45E-7& 1.3& 500        & 05:38:41.218 & -69:02:58.35 &G  & 0.02 &  86084583863296 & 8968085 &053841.212-690258.34 &C22           &  & O6.5IV((fc))+O6.5V((fc)), SB2 & Walborn & \\ % good match
  c6701    &  61& 1.32E-7& 1.1&1014        & 05:38:41.509 & -69:06:00.97 &G  & 0.1  &  85534828236416 &         &053841.507-690600.92 &C22           & S99-056 & O2-4.5+mid/lateO & HB12 & \\ % good match
  p1\_749  & 113& 3.68E-7& 1.1& 506        & 05:38:41.556 & -69:05:19.49 &G  & 0.05 &  85534828092032 & 9019926 &053841.545-690519.43 &C22           & Mk 25, P93-0871, S99-019,  & ON2V((n))((f*)), SB1s & Walborn & \\ % good match
  p1\_752 &54076& 1.46E-4& 1.5& 507        & 05:38:41.601 & -69:05:13.45 &G  & 0.05 &  85569167442432 &         &053841.601-690513.43 &C22 T19       & Brey 87, R140N [Mk], R140a [M87], S99-006, BAT99-101  +  102. See T19. & WC4(+WN6+O) & Evans &  ACIS pile-up \\ %good match; R140a
  p1\_754  & 396& 1.51E-6& 1.7& 509        & 05:38:41.625 & -69:05:15.18 &G  & 0.03 &  85569188005248 &         &053841.613-690515.17 &C22 T19       & Brey 87, R140S [Mk], R140b [M87], S99-008, BAT99-103. See T19. & WN5h(h)+O(+earlyO) & Evans & \\ %good match; R140b
  p1\_760  &  71& 1.75E-7& 1.2& 512        & 05:38:41.741 & -69:06:25.08 &G  & 0.01 &  79655028521472 &         &053841.734-690625.01 &C22           & P93-0885, S99-068 & O2V-III((f*)), SB1l & Walborn & \\ % good match
  p1\_786  & 194& 4.99E-7& 1.5&1017        & 05:38:41.870 & -69:06:14.49 &G  & 0.03 &  79659312965632 &         &053841.862-690614.41 &C22           & S99-088 & O2If*/WN5 & CW11 & \\ %good match; useful figure to demonstrate crowded extraction
  p1\_795  & 157& 3.54E-7& 1.2&1019        & 05:38:42.009 & -69:06:07.63 &G  & 0.04 &  79659292338176 &         &053842.004-690607.56 &C22           & S99-070 & O3III(f*)+O8 & MH98 & \\ % good match
  c6973    &  38& 1.50E-7& 1.3&1021        & 05:38:42.079 & -69:06:14.37 &G  & 0.15 &  79659312965248 &         &053842.072-690614.32 &C22           & S99-025 & O4If* & MH98 & \\ % good match
  c6974    & 161& 3.84E-7& 1.5& 522        & 05:38:42.088 & -69:05:45.54 &G  & 0.04 &  85534807590784 & 9019972 &053842.082-690545.47 &C22           & S99-134 &  &  & \\ % good match
  c7031    &  27& 6.85E-8& 1.9& 526        & 05:38:42.243 & -69:08:32.35 &G  & 0.23 &  79487513122048 & 9015834 &053842.238-690832.29 &C22           & P93-0925 & O8.5I((n))fp, SB1l & Walborn & \\ % good match
  p1\_830  &1680& 4.19E-6& 1.4& 527        & 05:38:42.359 & -69:04:58.19 &G  & 0.06 &  85564856502528 & 9019909 &053842.351-690458.19 &C22           & R139, Brey 86, P93-0952, S99-002 , BAT99-107 & O6.5Iafc+O6Iaf & T11 & \\ % good match
  c7131    &  90& 2.31E-7& 1.5&1022        & 05:38:42.403 & -69:06:15.14 &G  & 0.15 &  79659312957312 &         &053842.397-690615.08 &C22           & Mk 37, S99-028 & O4If* & MH98 & \\ % good match
  c7254    &  21& 6.66E-8& 1.2& 532        & 05:38:42.663 & -69:06:35.89 &G  & 0.09 &  79659311801600 & 8997593 &053842.657-690635.83 &C22           & P93-0974, S99-104 & O3V(n)((f*))z+OB, SB1l/SB2? & Walborn & \\ % good match
  p1\_893  &6955& 1.69E-5& 1.8&1025        & 05:38:42.903 & -69:06:04.96 &G  & 0.02 &  85534828237440 &         &\nodata              &C22 T19       & R136c; Blend of S99 027 \& 063. See T19. & WN5h & CD98 & \\ % good match
  c7410    &  69& 1.50E-7& 1.3&1026        & 05:38:43.060 & -69:06:11.26 &G  & 0.09 &  79659312979200 &         &\nodata              &C22           & Blend of S99 076 \& 191 & O2-4.5+mid/lateO & HB12 & ACIS aperture includes Doran725\_dM (distinct from VFTS src in HTTP image)\\ %good match; 
  p1\_911  & 204& 4.63E-7& 1.5& 542        & 05:38:43.097 & -69:05:46.89 &G  & 0.05 &  85530496766336 &         &053843.080-690546.86 &C22 T19       & Mk 30, P93-1018, S99-024, BAT99-113; also observed in Field A5 of the IFU data. See T19. & O2If*/WN5+lateO/earlyB & Evans & \\ % good match
  p1\_924  & 261& 5.70E-7& 1.5& 545        & 05:38:43.208 & -69:06:14.51 &G  & 0.07 &  79659312999296 &         &053843.202-690614.44 &C22 T19       & Mk 35, P93-1029, S99-023; also observed in Field A3 of the IFU data. See T19. & O2If*/WN5 & CW11 & \\ % good match
  p1\_937  &  39& 8.65E-8& 0.9&1028        & 05:38:43.268 & -69:06:16.58 &G  & 0.19 &  79659312998144 &         &053843.263-690616.51 &C22           & Mk 35S, S99-037 & O3.5-4.5 & HB12 & \\ % good match
  c7528    &  21& 5.00E-8& 1.4&1029        & 05:38:43.350 & -69:05:47.62 &G  & 0.38 &  85534807652224 &         &053843.343-690547.55 &C22           & S99-087 &  &  & marginal match: Gpos well outside Aerrbx\\
  c7552    &  26& 6.43E-8& 1.2&1030        & 05:38:43.423 & -69:05:42.08 &G  & 0.17 &  85534828273024 &         &\nodata              &C22           & S99-335 &  &  & \\ % good match
  p1\_955  & 116& 2.77E-7& 1.1&1031        & 05:38:43.688 & -69:05:47.93 &G  & 0.09 &  85534807650304 &         &053843.684-690547.89 &C22           & S99-039 & O3V & MH98 & \\ % good match
  c7859    &  27& 1.39E-7& 1.4& 562        & 05:38:44.413 & -69:05:36.25 &G  & 0.04 &  85530545537920 & 9019947 &053844.406-690536.22 &C22           & Mk 26, P93-1150, S99-032 &  &  & \\ % good match
  p1\_1021 &  24& 8.15E-8& 1.1& 564        & 05:38:44.559 & -69:05:12.42 &G  & 0.09 &  85564905241856 & 9020062 &053844.553-690512.35 &C22           & S99-253 & O6-8V((f)) & Walborn & \\ % good match
  c7907    &  48& 1.33E-7& 1.5& 566        & 05:38:44.569 & -69:04:51.25 &G  & 0.12 &  85569187906048 & 9019906 &053844.558-690451.19 &C22           & Mk 23, P93-1163, S99-042 & O3III(f*) & Walborn & \\ % good match
  cc5383   &  19& 9.77E-8& 1.5& 579        & 05:38:44.975 & -69:05:07.75 &G  & 0.09 &  85569187903104 &         &053844.969-690507.65 &C22           & In 'Knot 1' [WB87]; P93-1201, S99-171 & O9:((n)), SB?,VM2 & Walborn & \\ % good match
  c8052    &  22& 5.45E-8& 1.2& 585        & 05:38:45.272 & -69:05:46.61 &G  & 0.3  &  85534807640832 &         &053845.279-690546.53 &C22           & P93-1231, S99-031; also observed in Field A5 of the IFU data & O7V(n), SB1l,VM2 & Walborn & \\ % good match
  c8112    &  54& 1.43E-7& 1.3& 591        & 05:38:45.692 & -69:06:22.56 &G  & 0.04 &  79659311713024 &         &053845.687-690622.49 &C22           & Mk 12, P93-1257, S99-011 & B0.2Ia & McEvoy & \\ % good match
  c8160    &  64& 1.65E-7& 1.1& 599        & 05:38:46.183 & -69:06:17.47 &G  & 0.2  &  85534828283904 & 9020021 &053846.177-690617.39 &C22           & P93-1311, S99-040 & O3III(f*), SB1s & Walborn & \\ % good match
  p1\_1062 &  32& 8.67E-8& 1.4& 601        & 05:38:46.286 & -69:05:59.40 &G  & 0.13 &  85534828217856 & 9019999 &053846.280-690559.32 &C22           & Mk 14N, P93-1317, S99-091 & O5-6V((n))z & Walborn & \\ % good match
  c8180    &  22& 5.40E-8& 1.2& 603        & 05:38:46.539 & -69:04:28.04 &G  & 0.23 &  85672267222144 & 9019893 &053846.529-690427.99 &C22           & Mk 10, P93-1341 & O4III(fc), SB1l & Walborn & \\ % good match
  c8204    &  24& 6.38E-8& 1.1& 608        & 05:38:46.791 & -69:06:03.18 &G  & 0.24 &  85534828230528 & 9020002 &053846.785-690603.10 &C22           & Mk 14, P93-1350, S99-064 & O4III(f), SB1l & Walborn & \\ % good match
  p1\_1088 & 693& 1.74E-6& 1.4& 617        & 05:38:47.522 & -69:00:25.28 &G  & 0.23 &  87733851287040 & 8944472 &053847.533-690025.23 &C22 T19       & HDE 269926, R146, Sk-69 245, Brey 88, BAT99-117, P93-9033. See T19. & WN5ha & Evans & \\ % good match
  c8320    &  17& 6.79E-8& 1.8& 621        & 05:38:48.098 & -69:04:42.28 &G  & 0.18 &  85667984452864 & 9019899 &053848.089-690442.18 &C22           & In 'Knot 2' [WB87]; P93-1429 & O2V((f*))z,VM3 & Walborn & \\ % good match
  cc5800   &   6& 1.76E-8& 0.9& 640        & 05:38:49.665 & -69:08:54.84 &G  & 0.45 &  79418793663232 & 9019102 &053849.664-690854.73 &C22           & P93-1489 &  &  & \\ % good match
  c8591    &  24& 6.29E-8& 1.0& 648        & 05:38:50.407 & -69:05:38.26 &G  & 0.45 &  85500468549248 & 8989552 &053850.400-690538.17 &C22           & Mk 08, P93-1531, S99-058 & O5.5IV(f) & Walborn & marginal match: Gpos well outside Aerrbx, but nothing else closer\\
  p1\_1186 & 152& 4.02E-7& 1.4& 664        & 05:38:52.728 & -69:06:43.24 &G  & 0.02 &  85466108826624 & 9018610 &053852.724-690643.13 &C22           & Mk 04, P93-1607, S99-065 & O7II(f), SB? & Walborn & \\ % good match
  p1\_1234 & 302& 7.14E-7& 2.1& 682        & 05:38:55.527 & -69:04:26.80 &G  & 0.03 &  85637907503744 & 8979450 &053855.519-690426.72 &C22 T19       & P93-1732. See T19. & WN5h & Evans & \\ % good match
  p1\_1256 & 784& 1.87E-6& 2.0& 695        & 05:38:57.072 & -69:06:05.65 &G  & 0.06 &  85500468567040 & 9018590 &053857.072-690605.58 &C22 T19       & HDE 269928, R145, Sk-69 248, Brey 90, P93-1788, BAT99-119. See T19. & WN6h+? & Evans & \\ % good match
  p1\_1274 &   4& 1.05E-8& 3.3& 703        & 05:38:58.564 & -69:07:52.59 &G  & 0.63 &  79556232625408 & 9018687 &053858.561-690752.46 &C22           & P93-1828 & O7:V:+O8:V:, SB2 & Walborn & \\ % good match
  c10098   &  17& 4.01E-8& 1.3& 746        & 05:39:07.328 & -69:07:46.07 &G  & 0.63 &  79384433945344 & 9008310 &053907.327-690745.93 &C22           &  & O6Vnn & Walborn & VFTS src outside Aerrbx\\
  c10271   &  31& 7.36E-8& 1.2& 755        & 05:39:10.921 & -69:06:13.73 &G  & 0.25 &  85397389373184 & 8994892 &053910.913-690613.63 &C22           & P93-2041 & O3Vn((f*)) & Walborn & VFTS src just outside Aerrbx; \\ % good match
  c10289   &  99& 3.13E-7& 2.5& 758        & 05:39:11.324 & -69:02:01.56 &G  & 0.38 &  85977170493568 & 8960269 &\nodata              &C22 T19       & HD38344, R147, Sk-69 251, Brey 92, BAT99-122. See T19. & WN5(h) & Evans & VFTS src just outside Aerrbx; \\ % good match
  cc7769   &   5& 1.50E-8& 0.7& 768        & 05:39:16.235 & -69:01:20.38 &G  & 0.67 &  87493333392256 & 8958260 &\nodata              &C22           &  & O8Vn,NC & Walborn & \\ % good match
  cc7873   &   0& 1.79E-9& 4.2& 774        & 05:39:18.679 & -69:07:47.35 &G  & 1.03 &  85191230965760 & 9014727 &053918.676-690747.25 &C22           &  & O7.5IVp+O8.5:V:, SB2/SB3? & Walborn & \\ % good match
  p1\_1530 &  26& 6.68E-8& 0.9& 830        & 05:39:39.752 & -69:04:30.30 &G  & 0.35 &  82854768769024 & 9014580 &\nodata              &C22           & P93-2270 & O5-6V(n)((f)), SBl & Walborn & \\ 
  \\
\hline
\hline
\multicolumn{12}{l}{\bf\footnotesize Declared Counterparts in Doran13 Catalog}\\
  p1\_296 &1174 & 2.80E-6& 1.9& 185  & 05:37:49.039 & -69:05:08.21 &G   & 0.12 & 92338057418624 & 8986916 &053749.028-690508.33&C22 T19       & RMC 130. See T19.& WN/C+B1I & BAT99 & \\ % good match
  c4012   &  30 & 6.87E-8& 1.0& 273  & 05:38:13.162 & -69:05:36.41 &G   & 0.29 & 80655744058112 & 8991351 &053813.159-690536.51&              &                  &  &  & \\ % good match
  c5695   &  13 & 4.13E-8& 1.1& 398  & 05:38:36.243 & -69:06:08.46 &G   & 0.52 & 80415225947776 &         &053836.237-690608.42&C22           &                  &  &  & marginal match:  Doran src $\sim$0.4\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c5867   &  17 & 5.42E-8& 1.5& 415  & 05:38:37.438 & -69:05:50.34 &G   & 0.42 & 80415227189632 &         &053837.429-690550.30&              &                  &  &  & marginal match:  Doran src $\sim$0.4\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c5984   &  38 & 9.11E-8& 1.5& 427  & 05:38:38.454 & -69:04:17.98 &G   & 0.4  & 86423899131008 & 9019890 &053838.438-690417.94&C22           &                  & O8/9V & Bosch & \\ % good match
  c6062   &  65 & 1.92E-7& 2.8& 443  & 05:38:39.149 & -69:06:21.29 &G   & 0.1  & 79654981424640 & 9020032 &053839.143-690621.24&C22 T19       & Mk 49. See T19.  & WN6(h) & BAT99 & \\ % good match
  cc4651  &  41 & 9.88E-8& 1.7& 458  & 05:38:39.621 & -69:05:59.39 &G   & 0.16 & 79659312981760 & 9020000 &053839.614-690559.35&C22           &                  &  &  & \\ % good match
  c6164   &  10 & 4.51E-8& 1.2& 462  & 05:38:39.698 & -69:06:24.05 &G   & 0.32 & 79654981425664 & 9020034 &053839.692-690624.01&C22           &                  & O7III & Bosch & Doran462 (Gpos) between c6164,c6138 (just outside Aerrbx of c6164)\\
  c6170   &  22 & 7.69E-8& 1.4& 461  & 05:38:39.699 & -69:06:08.59 & D+ & 0.22 &                &         &053839.700-690608.63&C22           &                  &  &  & \\ % good match
  c6213   &  23 & 8.53E-8& 1.2& 472  & 05:38:39.853 & -69:06:09.55 &G   & 0.07 & 79659312983296 &         &053839.846-690609.50&C22           &                  &  &  & \\ % good match
  p1\_695 &  62 & 1.47E-7& 1.5& 475  & 05:38:40.150 & -69:05:51.31 &G   & 0.18 & 85530496759552 & 9019980 &053840.143-690551.26&C22           &                  & O3-6V & MH98 & \\ % good match
  p1\_711 & 124 & 3.49E-7& 1.5& 497  & 05:38:40.710 & -69:05:56.97 & D+ & 0.02 &                &         &053840.712-690556.99&              &                  &  &  & \\ % good match
  c6443   &  45 & 1.54E-7& 1.2& 502  & 05:38:40.805 & -69:05:25.15 &G   & 0.05 & 85534828067712 & 9019933 &053840.798-690525.10&C22           &                  & O5/6V & Bosch & \\ % good match
  p1\_718 &  45 & 1.23E-7& 1.3& 507  & 05:38:40.898 & -69:05:55.90 & D+ & 0.41 &                &         &053840.895-690555.93&C22           &                  &  &  & pretty good match; Doran src $\sim$0.4\arcsec away, well outside Aerrbx, but nothing else much closer\\
  c6472   &  22 & 7.76E-8& 1.2& 508  & 05:38:40.950 & -69:05:55.11 & D+ & 0.18 &                &         &053840.949-690555.14&C22           &                  &  &  & \\ % good match
  c6555   &  32 & 7.51E-8& 1.7& 521  & 05:38:41.150 & -69:05:49.45 &G   & 0.17 & 85534828224000 &         &053841.142-690549.40&              &                  &  &  & \\ % good match
  p1\_745 & 473 & 1.04E-6& 1.4& 539  & 05:38:41.488 & -69:05:56.89 & D+ & 0.08 &                &         &053841.490-690556.90&C22           &                  & O3V & MH98 & \\ % good match
  c6981   & 336 & 1.10E-6& 1.4& 576  & 05:38:42.079 & -69:06:02.22 & D+ & 0.08 &                &         &053842.081-690602.22&C22           &                  & O3V+O3-5V & MH98 & \\ % good match
  p1\_812 & 933 & 2.02E-6& 1.5& 580  & 05:38:42.112 & -69:05:55.33 &G   & 0.06 & 85534828234496 &         &053842.104-690555.29&C22           & Mk 42            & O2If* & CW11 & 3 other Doran srcs (573, 577, 587) in ACIS aperture, but this is definitely the best match\\ %good match; 
  cc4987  &  35 & 1.45E-7& 1.5& 604  & 05:38:42.259 & -69:06:00.46 & D+ & 0.13 &                &         &053842.258-690600.47&              &                  &  &  & \\ % good match
  cc4968  &  66 & 1.72E-7& 1.6& 612  & 05:38:42.308 & -69:06:04.94 & D+ & 0.2  &                &         &\nodata             &C22           &                  &  &  & in R136; dM position for Doran612; Doran600\_dM also in ACIS aperture\\
  c7109   &  36 & 1.67E-7& 2.6& 636  & 05:38:42.389 & -69:06:00.08 & D+ & 0.19 &                &         &053842.383-690600.09&              &                  &  &  & uncataloged HTTP source matches Asrc; Doran636 is just outside Aerrbx; in R136\\
  c7235   &   7 & 4.69E-8& 0.9& 677  & 05:38:42.623 & -69:05:36.79 &G   & 0.1  & 85534828074624 & 9020078 &053842.616-690536.74&C22           &                  & O6/7V((f)) & Bosch & \\ % good match
  p1\_867 & 522 & 1.61E-6& 1.4& 682  & 05:38:42.658 & -69:06:02.91 & D+ & 0.02 &                &         &\nodata             &C22           &                  & O3If* & MH98 & Doran682 uses dM position\\ %good match; 
  p1\_979 &2180 & 4.70E-6& 1.4& 765  & 05:38:44.129 & -69:05:56.71 &G   & 0.03 & 85534828260608 &         &053844.123-690556.63&C22           & Mk 33 Sa         & O3III(f*) & MH98 & \\ % good match
  p1\_995 &74445& 1.48E-4& 1.8& 770  & 05:38:44.256 & -69:06:06.00 &G   & 0.04 & 85534828257792 & 9020003 &053844.252-690605.93&C22 P18       & MK 34. See P18.  & WN5h & CD98 & ACIS pile-up \\ %good match; 
  p1\_1000&1865 & 4.09E-6& 1.5& 775  & 05:38:44.334 & -69:05:54.72 &G   & 0.02 & 85534828252672 &         &053844.329-690554.66&C22           & Mk 33 Na         & O3If* & MH98 & \\ % good match
  p1\_1033&  95 & 2.22E-7& 1.4& 800  & 05:38:44.958 & -69:05:54.18 &G   & 0.14 & 85534807639808 & 9020069 &053844.950-690554.11&C22           &                  & O3V & MH98 & \\ % good match
  c8022   &  16 & 5.78E-8& 2.2& 807  & 05:38:45.071 & -69:05:09.59 & D+ & 0.22 &                &         &053845.051-690509.73&              &                  &  &  & \\ % good match
  p1\_1035&  49 & 2.10E-7& 1.7& 810  & 05:38:45.148 & -69:05:08.46 &G   & 0.18 & 85564905253504 &         &053845.150-690508.34&C22           &                  & O3-6V & WB97 & \\ % good match
  p1\_1194&1233 & 2.90E-6& 1.8& 916  & 05:38:53.383 & -69:02:00.88 &G   & 0.1  & 86222022977920 & 8959289 &053853.363-690200.88&C22 T19       & RMC 144. See T19.& WN6h & BAT99 & \\ % good match
  cc8189  &  15 & 3.74E-8& 1.7& 1038 & 05:39:25.332 & -69:09:12.99 &G   & 1.09 & 76356437382656 & 9022508 &053925.334-690912.93&              &                  &  &  & \\ 
  \enddata
\tablecomments{
Reported properties of ACIS sources (NetCounts\_t, PhotonFlux\_t, MedianEnergy\_t from Table~\ref{xray_properties.tbl}) are derived by combining all observations.  In some cases the source detection is most significant in a single observation.
NetCounts suggests the quality of the extracted spectrum, but is unsuitable for photometry.  Apparent Photon Flux (NetCounts / MeanEffectiveArea / ExposureTimeNominal) is a rough scaling of NetCounts to account for source-to-source variations in exposure time, effective area, and aperture size \citep[][\S7.4]{Broos10}.
}
%
%\tablenotetextbox{a}{8in}{
\tablenotetext{a}{
The coordinates published in the VFTS and Doran catalogs were not directly used to assess positional coincidence between X-ray sources and candidate/known massive stars.
When the star could be identified in the Gaia catalog (Src ``G''), Gaia coordinates (propagated to the mean epoch of the \Chandra\ data, Y2014.5) and uncertainties were adopted.
Otherwise, when the star could be identified in the VMC catalog (Src ``V''), VMC coordinates were adopted and uncertainties were estimated by the authors.
Otherwise, pubished VFTS coordinates (``V+ '') were corrected using a field distortion map derived using Gaia and uncertainties were estimated by the authors.
Otherwise, published Doran coordinates (``D+ '') were corrected using frame shifts derived using Gaia and uncertainties were estimated by the authors.\\
}
%\vspace*{3em}
\tablenotetextbox{b}{8in}{
Separation between ACIS source and star's Adopted Coordinates; median is 0.15 arcsec.
}
\tablenotetextbox{c}{8in}{
Source label in the HTTP catalog.  Due to space limitations, our corrected HTTP positions are not reported.
}
\tablenotetextbox{d}{8in}{
Modeling of the T-ReX spectrum is described by 
\citet[C22]{Crowther22},
\citet[T19]{Tehrani19},
\citet[P18]{Pollock18},
\citet[C15]{Clark15}.
}
\tablenotetextbox{e}{8in}{
We suspect that the identifiers VFTS416 and Doran390 refer to the same star.
}
\tablenotetextbox{f}{8in}{
We suspect that the identifiers VFTS468 and Doran451 refer to the same star.
}
%\tablecomments{Spectral Type References: 
%(1) Evans et al. 2011; (2) Foellmi et al. (2003); (3) Crowther \& Smith (1997); (4) Smith et al. (1990); (5) Conti \& Massey (1989); (6) Crowther \& Dessart (1998); (7) Bartzakos et al. (2001); (8) Moffat et al. (1987); (9) Massey \& Hunter (1998); (10) Smith et al. (1996); (11) Schmutz \& Vacca (1991); (12) Crowther \& Hadfield (2006); (13) Walborn et al. (1999); (14) Torres-Dodgen \& Massey (1988); (15) de Koter et al. (1997), (16) Breysacher (1986); (17) De Marchi et al. (2011); (18) Schnurr et al. (2008).
%}
\end{deluxetable}
\end{longrotatetable}

==> no_clear_match.tex <==
%\documentclass[preprint,11pt,trackchanges]{aastex63}
%
%\usepackage{grffile}  %grffile allows .'s in filenames
%\usepackage{url}
%\begin{document}

% Reduce the space between table columns.
\setlength{\tabcolsep}{1mm}

%\begin{longrotatetable}
\startlongtable
\begin{deluxetable*}{@{}lrhp{5.5in}l@{}}
\tablecaption{Selected Candidate and Known Massive Stars Not Consistent With 1910 X-ray Sources Defined in Table~\ref{tbl:OIR_catalogs} \label{tbl:near_misses}
}
%\movetableright=-1in
%\movetabledown=1in
\tablewidth{10in}
\tabletypesize{\scriptsize}
\tablecolumns{13}
\tablehead{   
 \colhead{Label} &
 \colhead{NetCt} &
 \nocolhead{Possible Match} &
 \colhead{Comment}
 \\
 \colhead{} &
 \colhead{ct} &
 \colhead{} &
 \colhead{} 
}
%\colnumbers
\startdata                                                                                       
% REPORTED IN DORAN TABLE.
%  p1\_987 & 84 &  & VFTS1034 0.2\arcsec away (Gpos); Doran772\_dM 0.3\arcsec away; both could contribute to ACIS light\\
%  p1\_866 & 62 &  & Doran685 is 0.25\arcsec away (Gpos); Doran671\_dM is 0.5\arcsec away; both could contribute to ACIS light\\
%  p1\_832 & 4452 & Doran 633,630,642,638 & mushroom aperture at ACIS aimpoint; hopelessly confused at R136 core\\
%  p1\_766 & 31 &  & VFTS513 0.2\arcsec away (Gpos); VFTS515 0.4\arcsec away (NOT Gpos); both could contribute to ACIS light\\
%  cc4970 & 496 & Doran 613,621 & in R136; $\sim$8 Doran srcs in ACIS aperture\\
%  c7182 & 258 & Doran 657,652,649,659 & many Doran sources in ACIS aperture; in R136\\
%  c7157 & 345 & Doran 648,624 & many Doran sources in ACIS aperture; in R136\\
%  c7018 & 45 & Doran 589,583 & many Doran sources in ACIS aperture; in R136\\
%
p1\_988 & 28 &  & VFTS1032 \& VFTS1035 $\sim$1\arcsec away (Gpos); both well outside Aerrbx; no HTTP light on ACIS src, but HTTP \#415625 nearby\\
 cc8528 & -9 & NONE & Doran1061 $\sim$1.4\arcsec away (Gpos), not too far outside Aerrbx; no HTTP light on ACIS src\\
 cc8242 & 15 & NONE & VFTS791 $\sim$1.1\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src, but \#283782 nearby\\
 cc6978 & 14 & NONE & VFTS728 $\sim$0.8\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
 cc6015 & 10 & NONE & VFTS659 $\sim$0.9\arcsec away (Gpos), well outside Aerrbx; HTTP streak goes through Asrc\\
 cc5386 &  5 & NONE & VFTS582 $\sim$0.9\arcsec away, well outside Aerrbx; HTTP \#421776 matches Asrc\\
 cc5097 & 22 & NONE & Doran702 $\sim$0.8\arcsec away (Gpos), well outside Aerrbx; much fainter HTTP \#450187 matches Asrc\\
 cc5042 & 17 & NONE & Doran666 $\sim$1\arcsec away (Gpos), well outside Aerrbx; much fainter HTTP \#298765 matches Asrc\\
 cc4973 & 18 & NONE & VFTS524 $\sim$1\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
 cc4926 & 92 & VFTS 1015 & VFTS1015 $\sim$0.6\arcsec away (NOT Gpos) near HTTP \#407456, well outside Aerrbx; several closer HTTP sources\\
 cc4730 & 10 & NONE & VFTS484 $\sim$0.9\arcsec away (Gpos), well outside Aerrbx; several closer HTTP sources\\
 cc4590 &  4 & NONE & VFTS452 $\sim$1.4\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
 cc4566 &  1 & NONE & VFTS449 $\sim$0.7\arcsec away (Gpos), well outside Aerrbx\\
 cc3076 & 11 & NONE & VFTS311 0.9\arcsec away (Gpos), well outside Aerrbx; faint un-IDd HTTP src very near ACIS src\\
  cc220 & -7 & NONE & Doran79 2.6\arcsec away (Gpos), well outside Aerrbx; many Gaia srcs nearby; no VMC Yband light on ACIS src\\
 cc1675 & 79 & NONE & VFTS216 $\sim$1.3\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c8147 & 40 & NONE & VFTS600 $\sim$1.1\arcsec away (Gpos), well outside Aerrbx; diffuse HTTP light on ACIS src\\
  c8111 & 29 & NONE & VFTS586 $\sim$1\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c7519 & 69 & NONE & Doran745 $\sim$0.8\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c7452 &124 &      & ACIS src matches fainter HTTP src, not Doran732\_dM,734\_dM, well outside Aerrbx\\
  c7393 & 12 & NONE & Doran708 $\sim$0.7\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
   c713 &196 &      & ACIS position 1.6\arcsec west of VFTS2; ACIS aperture includes VFTS3\\
  c7115 & 63 & NONE & ACIS src matches fainter HTTP src, not Doran639\_dM $\sim$0.7\arcsec away, well outside Aerrbx\\
  c7055 & 20 & NONE & Doran588 (Gpos) $\sim$0.7\arcsec away, well outside Aerrbx; several closer HTTP sources\\
  c6962 & 28 & NONE & Doran574 (Gpos) $\sim$0.7\arcsec away, well outside Aerrbx; several closer HTTP sources\\
  c6563 & 22 & NONE & ACIS src matches fainter HTTP src, not VFTS1006 (Gpos) aka Doran511 0.7\arcsec away\\
  c6187 & 11 & NONE & Doran457\_S $\sim$0.8\arcsec away, well outside Aerrbx; several closer HTTP sources\\
  c6184 & 10 & NONE & Doran469 $\sim$0.8\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c6102 & 15 & NONE & Doran455\_dM 0.6\arcsec away, several closer HTTP sources\\
  c5306 & 10 & NONE & VFTS398 0.7\arcsec away (Gpos)\\
  c5109 &  2 & NONE & Doran351 0.8\arcsec away (Gpos), no HTTP light on ACIS src\\
  c3274 & 47 & NONE & Doran216 $\sim$5\arcsec away\\
  c1308 & 11 &      & VFTS91 $\sim$1.2\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c1245 & 87 &      & VFTS72 $\sim$1.5\arcsec away (Gpos), well outside Aerrbx; no VMC Yband light on ACIS src\\
  c1216 & 37 &      & VFTS69 $\sim$1\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
  c1186 &102 &      & VFTS63 2\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src\\
 c10133 & 10 & NONE & VFTS749 $\sim$1\arcsec away (Gpos), well outside Aerrbx; no HTTP light on ACIS src
\enddata
\end{deluxetable*}
%\end{longrotatetable}

%\end{document}


==> other_counterparts.tex <==
% Reduce the space between table columns.
\setlength{\tabcolsep}{1mm}

\begin{longrotatetable}
\startlongtable
\begin{deluxetable}{@{}lcccccccrccccp{2.0in}@{}}
%\movetableright=-1in
\movetabledown=0.5in
\tablewidth{10in}
\tabletypesize{\tiny}
\tablecolumns{14}
\tablecaption{Counterparts To X-ray Sources Beyond the Massive Stellar Population \label{tbl:other_matches}}       
\tablehead{
 \multicolumn{2}{c}{X-ray Source} &
 \multicolumn{4}{c}{Gaia+VMC} &
 \multicolumn{4}{c}{HTTP\tablenotemark{a}} &
 \multicolumn{3}{c}{SAGE} &
\\[-5pt]
 \multicolumn{2}{c}{\hrulefill} &
 \multicolumn{4}{c}{\hrulefill} &
 \multicolumn{4}{c}{\hrulefill} &
 \multicolumn{3}{c}{\hrulefill}
\\[-8pt]
 \colhead{Label} &
 \colhead{PosErr} &
%
 \colhead{Dist.\tablenotemark{b}} &
 \colhead{Gaia ID} &
 \colhead{VMC ID} &
 \colhead{K} &
%
 \colhead{Dist.\tablenotemark{b}} &
 \colhead{ID} &
 \colhead{Shift} &
 \colhead{F555} &
%
 \colhead{Dist.\tablenotemark{b}} &
 \colhead{SAGE ID} &
 \colhead{3.6\micron} &
 \colhead{SIMBAD\tablenotemark{c}}   % Cone search in SIMBAD done with 1" radius.
\\[-7pt]
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{} &
% \colhead{Cit\tablenotemark{bbb}} &
%\\[-7pt]
 \colhead{} &
 \colhead{\arcsec} &
 \colhead{\arcsec} &
 \colhead{\#4657} &
 \colhead{\#55834} &
 \colhead{mag} &
 \colhead{\arcsec} &
 \colhead{} &
 \colhead{mas} &
 \colhead{mag} &
 \colhead{\arcsec} &
 \colhead{} &
 \colhead{mag} 
}
%\colnumbers                     \nodata             
\startdata
%& Label     & PosErr& MatchDist\_2& designation& sourceID& ksAperMag3& MatchDist\_3& HTTP& Correction& F555\_clean& MatchDist\_4& SSTISAGEMA& [3\_6]&
%
% Associations asserted by human judgment (near-miss in automated matching).
  p1\_255     &     &     &                  &         &     &     &                     &              &     &     &                       &      & Pulsar (PSR~J0537-6910) \\
  pass52\_4   &     & 0.47& 783116463742336  & 8880341 & 10  &     &                       &            &     &     &                       &      & Rotationally variable Star (HD~269921) \\
% From automated matching.
% DATE-HDU: 2019-10-20T18:01:35
 c12211       & 0.7 &     &                  &         &     &     &                       &            &     & 1.4 &   J054131.00-690020.5 & 17   &  \\
 c12192       & 0.8 & 0.8 &                  & 8885859 & 15  &     &                       &            &     & 0.6 &   J054130.44-685350.8 & 15   &  High proper-motion Star (OGLE LMC182.8 3168)\\
 c12175       & 0.8 & 1.2 &  634132646994048 & 9056388 & 19  &     &                       &            &     &     &                       &      &  \\
 c12160       & 1.0 & 2.3 &  634506333763584 & 9032618 &     &     &                       &            &     &     &                       &      &  \\
 c12121       & 0.4 & 0.3 &                  & 9100361 & 16  &     &                       &            &     & 0.4 &   J054058.33-691709.9 & 16   &  \\
 c11905       & 0.3 &     &                  &         &     &     &                       &            &     & 0.5 &   J054023.51-685650.0 & 12   &   Eclipsing binary (OGLE LMC-ECL-22109)\\
 p1\_1562     & 0.2 &     &                  &         &     &     &                       &            &     & 0.5 &   J054022.13-690737.6 & 17   &  \\
 c11900       & 0.6 & 1.1 &                  & 9768025 & 19  &     &                       &            &     & 1.1 &   J054021.78-685804.4 & 18   &  \\
 c11874       & 0.4 & 0.8 &                  & 8993129 & 17  &     &                       &            &     & 0.6 &   J054019.90-690559.7 & 16   &  \\
 c11868       & 0.2 & 0.3 &                  & 8995316 & 18  &     &                       &            &     & 0.4 &   J054019.51-690616.4 & 16   &  \\
 c11799       & 0.2 & 0.4 &                  & 9128440 & 16  &     &                       &            &     &     &                       &      &  \\
 c11784       & 0.2 &     &                  &         &     &     &                       &            &     & 0.2 &   J054009.61-691035.1 & 16   &  \\
 c11771       & 0.2 & 0.3 &                  & 9773382 & 19  &     &                       &            &     &     &                       &      &  \\
 p1\_1559     & 0.2 & 0.3 &                  & 9770859 & 20  &     &                       &            &     &     &                       &      &  \\
 c11757       & 0.2 & 0.4 &                  & 9100726 & 12  &     &                       &            &     & 0.5 &   J054008.30-691712.5 & 12   &  \\
 c11744       & 0.2 & 0.2 &                  & 8957258 & 17  &     &                       &            &     & 0.2 &   J054006.31-690152.2 & 16   &  \\
 c11737       & 0.3 & 0.0 &                  & 9028189 & 17  &     &                       &            &     & 0.4 &   J054005.88-690949.5 & 16   &  \\
 p1\_1557     & 0.2 & 0.2 &                  & 9774112 & 19  &     &                       &            &     & 0.3 &   J054001.84-690618.4 & 17   &  \\
 pass51\_3    & 0.2 &     &                  &         &     &     &                       &            &     & 0.8 &   J054001.03-690642.1 & 17   &  \\
 p1\_1552     & 0.1 & 0.1 &                  & 8994562 & 16  &     &                       &            &     & 0.2 &   J053958.69-690610.5 &      &  \\
 c11517       & 0.6 &     &                  &         &     &     &                       &            &     & 1.5 &   J053956.76-685834.2 & 16   &  \\
 p1\_1548     & 0.2 & 0.4 &                  & 9712401 & 19  & 0.2 &  053955.602-690846.62 &   130,688  & 25  &     &                       &      &  \\
 pass52\_5    & 0.3 & 0.3 &                  & 8890736 & 18  &     &                       &            &     & 0.8 &   J053952.08-685424.3 & 17   &  \\
 c11420       & 0.2 &     &                  &         &     &     &                       &            &     & 0.3 &   J053951.47-690450.4 & 17   &  \\
 c11429       & 0.4 &     &                  &         &     &     &                       &            &     & 0.7 &   J053950.51-691635.5 & 14   &  \\
 c11362       & 0.2 & 0.2 &  682751669602432 & 8996234 & 17  &     &                       &            &     & 0.2 &   J053947.31-690622.1 & 16   &  \\
 pass52\_8    & 0.3 & 0.3 &                  & 9769468 & 20  &     &                       &            &     &     &                       &      &  \\
 c11303       & 0.1 &     &                  &         &     & 0.3 &  053943.960-690939.37 &   32,295   & 24  &     &                       &      &  \\
 c11294       & 0.2 & 0.1 &                  & 9707911 & 19  &     &                       &            &     &     &                       &      &  \\
 p1\_1533     & 0.1 &     &                  &         &     & 0.1 &  053940.190-690801.39 &   64,202   & 25  &     &                       &      &  \\
 p1\_1529     & 0.2 & 0.1 &  684980764259456 & 8944793 & 16  &     &                       &            &     & 0.2 &   J053939.44-690029.7 & 14   &  AGN ([GC2009] J053939.48-690030.0)\\
 c11125       & 0.3 & 0.2 &                  & 8919503 & 15  &     &                       &            &     & 0.1 &   J053938.25-685740.2 & 14   &  YSO (2MASS J05393821-6857404)\\
 p1\_1521     & 0.1 & 0.2 &  682923488239360 & 9014587 & 13  & 0.3 &  053935.478-690438.90 &   204,381  & 17  & 0.4 &   J053935.50-690438.6 & 12   &  \\
 cc8524       & 0.2 &     &                  &         &     & 0.4 &  053935.206-690622.26 &   113,191  & 24  &     &                       &      &  \\
 p1\_1520     & 0.1 & 0.1 &                  & 9708958 & 18  &     &                       &            &     & 0.5 &   J053934.47-690323.5 & 17   &  \\
 p1\_1517     & 0.2 & 0.3 &                  & 9778551 & 20  &     &                       &            &     & 0.5 &   J053933.97-691130.4 & 16   &  \\
 p1\_1500     & 0.1 &     &                  &         &     & 0.4 &  053931.573-690951.65 &   -14,10   & 24  &     &                       &      &  \\
 c10839       & 0.3 & 0.2 &                  & 9716092 & 18  &     &                       &            &     &     &                       &      &  \\
 cc8372       & 0.2 &     &                  &         &     & 0.3 &  053929.424-690418.56 &   167,231  & 21  &     &                       &      &  \\
 c10813       & 0.2 &     &                  &         &     & 0.1 &  053928.754-690552.55 &   98,100   & 25  &     &                       &      &  \\
 cc8242       & 0.2 &     &                  &         &     & 0.4 &  053926.358-690522.78 &   112,102  & 23  &     &                       &      &  \\
 c10740       & 0.3 & 0.5 &                  & 9713682 & 18  & 0.2 &  053925.779-691031.35 &   -28,-54  & 23  &     &                       &      &  \\
 cc8125       & 0.3 &     &                  &         &     & 0.6 &  053924.343-691117.23 &   -26,-34  & 23  &     &                       &      &  \\
 cc8140       & 0.2 &     &                  &         &     & 0.3 &  053924.138-690520.12 &   108,83   & 24  &     &                       &      &  \\
 cc8012       & 0.2 &     &                  &         &     & 0.2 &  053921.754-690822.45 &   6,-73    & 24  &     &                       &      &  \\
 cc7981       & 0.2 &     &                  &         &     & 0.3 &  053921.352-690514.59 &   88,17    & 24  &     &                       &      &  \\
 c10571       & 0.1 & 0.2 &                  & 9020418 & 18  &     &                       &            &     &     &                       &      &  \\
 c10534       & 0.2 & 0.4 &                  & 9774389 & 18  &     &                       &            &     &     &                       &      &  \\
 c10435       & 0.6 &     &                  &         &     &     &                       &            &     & 0.9 &   J053916.16-685047.7 & 17   &  \\
 c10422       & 0.2 & 0.2 &                  & 9768044 & 18  &     &                       &            &     & 0.2 &   J053915.91-685752.2 & 17   &  \\
 p1\_1420     & 0.2 & 0.3 &                  & 8939594 & 16  &     &                       &            &     & 0.6 &   J053915.91-685950.0 & 15   &  \\
 c10393       & 0.2 & 0.1 &  679281354744320 & 9023693 & 14  & 0.1 &  053914.961-690923.81 &   -20,-139 & 19  & 0.1 &   J053914.96-690923.7 & 14   &  Long-period variable star (2MASS J05391496-6909238) \\
 c10378       & 0.1 & 0.2 &                  & 8997921 & 18  &     &                       &            &     &     &                       &      &  \\
 c10375       & 0.2 & 0.3 &                  & 9768536 & 19  &     &                       &            &     &     &                       &      &  \\
 c10370       & 0.2 & 0.1 &                  & 9767609 & 19  &     &                       &            &     & 0.1 &   J053913.96-685728.6 & 17   &  \\
 c10266       & 0.1 & 0.2 &  679384433817472 & 9014737 &     & 0.2 &  053910.764-690756.78 &   10,-129  & 18  & 0.4 &   J053910.79-690756.7 & 15   &  \\
 p1\_1391     & 0.0 & 0.1 &                  & 9773625 & 19  &     &                       &            &     &     &                       &      &  \\
 cc7435       & 0.2 &     &                  &         &     & 0.5 &  053910.220-690839.54 &   -3,-143  & 23  &     &                       &      &  \\
 c10215       & 0.2 &     &                  &         &     & 0.2 &  053909.980-690349.18 &   75,-13   & 23  &     &                       &      &  \\
 c10200       & 0.1 &     &                  &         &     & 0.2 &  053909.634-690606.06 &   46,-96   & 24  &     &                       &      &  \\
 c10129       & 0.4 &     &                  &         &     &     &                       &            &     & 0.6 &   J053908.87-685444.4 & 17   &  \\
 p1\_1368     & 0.1 & 0.1 &                  & 9706871 & 18  &     &                       &            &     & 0.1 &   J053908.45-685958.6 & 16   &  \\
 cc7254       & 0.1 &     &                  &         &     & 0.4 &  053907.078-690719.73 &   25,-128  & 23  &     &                       &      &  \\
 c10064       & 0.1 &     &                  &         &     & 0.5 &  053906.517-690946.39 &   -25,-147 & 23  &     &                       &      &  \\
 c10019       & 0.1 & 0.1 &  685844045425536 &         &     &     &                       &            &     &     &                       &      &  \\
 p1\_1340     & 0.0 & 0.1 &                  & 9771615 & 19  &     &                       &            &     &     &                       &      &  \\
 p1\_1317     & 0.0 & 0.0 &                  & 9774684 & 21  & 0.0 &  053903.176-690703.87 &   24,-125  & 24  &     &                       &      &  \\
 c9821        & 0.1 & 0.2 &                  & 8965678 &     &     &                       &            &     &     &                       &      &  \\
 p1\_1307     & 0.2 &     &                  &         &     &     &                       &            &     & 0.5 &   J053902.25-685847.7 & 16   &  \\
 c9590        & 0.2 & 0.3 &                  & 8938310 & 18  &     &                       &            &     & 0.4 &   J053859.69-685949.3 & 17   &  \\
 c9506        & 0.4 & 0.3 &                  & 8849680 & 17  &     &                       &            &     & 0.3 &   J053859.31-684959.5 & 15   &  \\
 p1\_1269     & 0.1 & 0.1 &                  & 9768987 & 19  &     &                       &            &     &     &                       &      &  \\
 c9251        & 0.1 &     &                  &         &     & 0.3 &  053856.961-690416.62 &   42,-81   & 23  &     &                       &      &  \\
 p1\_1246     & 0.2 & 0.4 &  688416745861760 & 8912946 & 17  &     &                       &            &     & 0.3 &   J053856.83-685636.3 & 15   &  \\
 c9209        & 0.1 & 0.1 &                  & 8978864 &     & 0.1 &  053856.710-690426.29 &   42,-84   & 22  &     &                       &      &  \\
 cc6320       & 0.1 &     &                  &         &     & 0.3 &  053855.594-690928.11 &   -9,-126  & 23  &     &                       &      &  \\
 c8856        & 0.0 &     &                  &         &     & 0.1 &  053853.098-690627.12 &   32,-99   & 25  &     &                       &      &  \\
 c8847        & 0.1 &     &                  &         &     & 0.4 &  053853.032-690433.13 &   39,-81   & 25  &     &                       &      &  \\
 cc6099       & 0.1 &     &                  &         &     & 0.4 &  053852.797-690614.66 &   34,-99   & 25  &     &                       &      &  \\
 c8790        & 0.1 & 0.2 &                  & 9707745 & 18  &     &                       &            &     & 0.2 &   J053852.25-690126.9 & 17   &  \\
 c8769        & 0.1 &     &                  &         &     & 0.1 &  053851.969-690602.04 &   34,-97   & 23  &     &                       &      &  \\
 cc5939       & 0.2 & 0.6 &                  & 9715032 & 17  &     &                       &            &     &     &                       &      &  \\
 cc5942       & 0.1 &     &                  &         &     & 0.2 &  053851.089-690612.33 &   34,-94   & 26  &     &                       &      &  \\
 c8646        & 0.2 &     &                  &         &     & 0.5 &  053850.870-691251.05 &   -14,-22  & 25  &     &                       &      &  \\
 c8464        & 0.0 & 0.3 &                  & 9023676 & 18  &     &                       &            &     &     &                       &      &  \\
 c8451        & 0.1 &     &                  &         &     & 0.0 &  053848.996-690358.58 &   36,-68   & 23  &     &                       &      &  \\
 cc5713       & 0.1 &     &                  &         &     & 0.4 &  053848.720-690715.56 &   27,-94   & 23  & 0.4 &   J053848.73-690715.6 & 15   &  \\
 cc5715       & 0.1 &     &                  &         &     & 0.3 &  053848.741-690615.44 &   36,-90   & 23  &     &                       &      &  \\
 c8426        & 0.1 &     &                  &         &     & 0.2 &  053848.774-690307.58 &   21,-61   & 18  &     &                       &      &  \\
 c8378        & 0.1 &     &                  &         &     & 0.0 &  053848.403-690603.96 &   36,-82   & 21  &     &                       &      &  \\
 c8342        & 0.1 &     &                  &         &     & 0.3 &  053848.240-690411.62 &   34,-64   & 24  &     &                       &      &  YSO (2MASS J05384813-6904117)\\
 c8337        & 0.1 &     &                  &         &     & 0.2 &  053848.105-690411.49 &   34,-64   & 24  &     &                       &      &  YSO (2MASS J05384813-6904117)\\
 c8313        & 0.1 &     &                  &         &     & 0.1 &  053848.041-690412.69 &   34,-64   & 23  &     &                       &      &  YSO (RRG 30 Dor N IRS 6)\\
 c8315        & 0.1 & 0.3 &                  & 9770921 & 18  &     &                       &            &     & 0.4 &   J053848.05-690210.8 & 16   &  \\
 c8248        & 0.1 &     &                  &         &     & 0.1 &  053847.281-690622.41 &   34,-84   & 22  &     &                       &      &  \\
 cc5551       & 0.1 &     &                  &         &     & 0.3 &  053847.189-690625.40 &   34,-84   & 23  &     &                       &      &  \\
 c8216        & 0.1 &     &                  &         &     & 0.2 &  053846.871-690505.58 &   38,-73   & 24  & 0.2 &   J053846.84-690505.4 & 10   &  \\
 cc5529       & 0.1 &     &                  &         &     & 0.2 &  053846.706-690554.95 &   36,-78   & 23  &     &                       &      &  \\
 c8146        & 0.1 &     &                  &         &     & 0.3 &  053846.132-690508.96 &   38,-73   & 23  &     &                       &      &  \\
 p1\_1057     & 0.1 & 0.1 &                  & 9778715 & 19  &     &                       &            &     &     &                       &      &  \\
 c8135        & 0.1 &     &                  &         &     & 0.2 &  053845.924-690518.53 &   38,-72   & 23  &     &                       &      &  \\
 p1\_1056     & 0.2 & 0.2 &                  & 8921036 & 18  &     &                       &            &     & 0.5 &   J053845.63-685759.7 &      &  \\
 c8058        & 0.1 &     &                  &         &     & 0.2 &  053845.251-690441.39 &   39,-67   & 25  &     &                       &      &  \\
 c7915        & 0.1 &     &                  &         &     & 0.0 &  053844.630-690405.04 &   31,-60   & 25  &     &                       &      &  \\
 cc5297       & 0.3 &     &                  &         &     & 0.8 &  053844.328-691203.28 &   -23,-45  & 24  &     &                       &      &  \\
 c7809        & 0.1 &     &                  &         &     & 0.2 &  053844.182-690541.30 &   35,-67   & 18  &     &                       &      &  Eclipsing binary (OGLE LMC-ECL-21456) \\
 cc5221       & 0.1 &     &                  &         &     & 0.2 &  053843.844-690646.02 &   33,-69   & 23  &     &                       &      &  \\
 cc5190       & 0.1 &     &                  &         &     & 0.1 &  053843.554-690550.38 &   37,-64   & 24  &     &                       &      &  \\
 c7568        & 0.1 & 0.1 &                  & 8996929 & 17  & 0.2 &  053843.546-690628.82 &   33,-69   & 18  & 0.4 &   J053843.50-690629.0 & 14   &  YSO (OGLE LMC-ECL-21448)\\
 c7590        & 0.0 &     &                  &         &     & 0.2 &  053843.555-690615.37 &   33,-68   & 19  &     &                       &      &  \\
 c7511        & 0.1 &     &                  &         &     & 0.1 &  053843.424-690538.52 &   42,-61   & 24  &     &                       &      &  \\
 c7519        & 0.0 &     &                  &         &     & 0.1 &  053843.299-690609.34 &   34,-68   & 23  &     &                       &      &  \\
 p1\_883      & 0.1 &     &                  &         &     & 0.3 &  053842.880-690556.46 &   39,-57   & 23  &     &                       &      &  \\
 cc5086       & 0.1 &     &                  &         &     & 0.2 &  053842.801-690545.39 &   39,-59   & 23  &     &                       &      &  \\
 c7239        & 0.1 &     &                  &         &     & 0.1 &  053842.629-690537.24 &   39,-60   & 18  &     &                       &      &  \\
 c7218        & 0.1 &     &                  &         &     & 0.4 &  053842.554-690421.41 &   33,-53   & 22  &     &                       &      &  \\
 cc5029       & 0.0 &     &                  &         &     & 0.3 &  053842.404-690559.19 &   36,-57   & 22  &     &                       &      &  \\
 c7115        & 0.0 &     &                  &         &     & 0.0 &  053842.341-690606.99 &   30,-62   & 22  &     &                       &      &  \\
 c7055        & 0.1 &     &                  &         &     & 0.2 &  053842.259-690624.81 &   35,-66   & 19  &     &                       &      &  \\
 c7032        & 0.1 &     &                  &         &     & 0.2 &  053842.165-690618.50 &   35,-62   & 22  &     &                       &      &  \\
 c6851        & 0.1 &     &                  &         &     & 0.2 &  053841.805-690552.67 &   37,-54   & 22  &     &                       &      &  \\
 cc4926       & 0.0 &     &                  &         &     & 0.3 &  053841.741-690603.93 &   27,-46   & 21  &     &                       &      &  \\
 cc4903       & 0.1 &     &                  &         &     & 0.1 &  053841.683-690617.07 &   36,-56   & 25  &     &                       &      &  \\
 c6631        & 0.1 &     &                  &         &     & 0.3 &  053841.303-690536.17 &   37,-55   & 24  &     &                       &      &  \\
 c6620        & 0.1 &     &                  &         &     & 0.4 &  053841.306-690649.85 &   33,-62   & 23  &     &                       &      &  \\
 c6503        & 0.1 &     &                  &         &     & 0.3 &  053841.040-690610.67 &   35,-54   & 20  &     &                       &      &  \\
 c6481        & 0.1 &     &                  &         &     & 0.2 &  053840.880-690611.28 &   35,-54   & 24  &     &                       &      &  \\
 c6373        & 0.1 &     &                  &         &     & 0.3 &  053840.520-690626.31 &   37,-53   & 25  &     &                       &      &  \\
 c6366        & 0.1 &     &                  &         &     & 0.2 &  053840.530-690534.03 &   39,-50   & 23  &     &                       &      &  \\
 cc4713       & 0.1 &     &                  &         &     & 0.2 &  053840.254-690540.36 &   39,-48   & 20  &     &                       &      &  \\
 c6248        & 0.1 &     &                  &         &     & 0.2 &  053839.956-690432.63 &   34,-38   & 21  &     &                       &      &  \\
 c6236        & 0.1 & 0.2 &                  & 9774528 & 17  & 0.2 &  053839.963-690652.52 &   33,-54   & 26  &     &                       &      &  \\
 p1\_686      & 0.1 & 0.2 &                  & 9778463 & 18  &     &                       &            &     &     &                       &      &  \\
 c6200        & 0.1 &     &                  &         &     & 0.2 &  053839.791-690613.57 &   36,-49   & 23  &     &                       &      &  \\
 c6150        & 0.1 & 0.0 &  685534828103552 &         &     & 0.0 &  053839.633-690532.25 &   39,-48   & 17  &     &                       &      &  \\
 c6135        & 0.1 &     &                  &         &     & 0.3 &  053839.523-690602.65 &   36,-50   & 24  &     &                       &      &  \\
 c6067        & 0.1 &     &                  &         &     & 0.0 &  053839.167-690609.08 &   35,-49   & 22  &     &                       &      &  \\
 c6071        & 0.1 &     &                  &         &     & 0.3 &  053839.158-690710.37 &   32,-53   & 25  &     &                       &      &  \\
 c6048        & 0.1 &     &                  &         &     & 0.3 &  053839.128-690548.30 &   38,-44   & 24  &     &                       &      &  \\
 c6020        & 0.1 &     &                  &         &     & 0.3 &  053838.769-690549.54 &   38,-44   & 24  &     &                       &      &  \\
 c6014        & 0.1 &     &                  &         &     & 0.4 &  053838.763-690528.56 &   39,-48   & 21  &     &                       &      &  \\
 c5995        & 0.1 & 0.2 &  679659312977664 &         &     & 0.2 &  053838.549-690612.85 &   35,-45   & 17  &     &                       &      &  \\
 c5962        & 0.1 &     &                  &         &     & 0.1 &  053838.316-690629.39 &   36,-45   & 19  &     &                       &      &  \\
 c5959        & 0.1 &     &                  &         &     & 0.2 &  053838.326-690552.36 &   37,-42   & 23  &     &                       &      &  \\
 c5954        & 0.1 & 0.1 &  686290742317824 &         &     &     &                       &            &     &     &                       &      &  \\
 cc4532       & 0.1 &     &                  &         &     & 0.2 &  053838.036-690521.21 &   38,-39   & 24  &     &                       &      &  \\
 p1\_657      & 0.1 &     &                  &         &     & 0.2 &  053837.596-690548.43 &   37,-41   & 23  &     &                       &      &  \\
 c5836        & 0.3 & 0.5 &                  & 9705089 & 17  &     &                       &            &     & 0.7 &   J053837.20-685655.0 & 16   &  \\
 p1\_641      & 0.2 & 0.2 &                  & 9767536 & 19  &     &                       &            &     & 0.3 &   J053836.65-685725.9 & 18   &  \\
 c5749        & 0.1 &     &                  &         &     & 0.4 &  053836.676-690525.80 &   37,-38   & 21  &     &                       &      &  \\
 p1\_639      & 0.1 & 0.2 &                  & 9038525 &     & 0.2 &  053836.577-691056.66 &   -14,-38  & 22  &     &                       &      &  \\
 c5683        & 0.1 &     &                  &         &     & 0.1 &  053836.307-690315.98 &   16,-27   & 23  &     &                       &      &  \\
 c5641        & 0.1 & 0.4 &  686836215582848 & 8963476 & 16  &     &                       &            &     &     &                       &      &  \\
 c5596        & 0.1 &     &                  &         &     & 0.2 &  053835.705-690525.58 &   38,-31   & 22  &     &                       &      &  \\
 c5512        & 0.1 &     &                  &         &     & 0.3 &  053835.144-690631.48 &   36,-39   & 24  &     &                       &      &  \\
 c5504        & 0.1 &     &                  &         &     & 0.1 &  053835.084-690556.99 &   38,-29   & 18  &     &                       &      &  \\
 p1\_629      & 0.1 & 0.3 &                  & 9768778 & 20  &     &                       &            &     &     &                       &      &  \\
 p1\_609      & 0.3 & 0.7 &                  & 8923829 & 18  &     &                       &            &     & 0.3 &   J053833.49-685817.9 & 17   &  \\
 cc4029       & 0.1 &     &                  &         &     & 0.4 &  053833.353-690755.97 &   28,-30   & 20  &     &                       &      &  \\
 c5274        & 0.1 &     &                  &         &     & 0.2 &  053832.944-690723.53 &   32,-28   & 24  &     &                       &      &  \\
 c5240        & 0.1 &     &                  &         &     & 0.3 &  053832.635-690555.07 &   40,-12   & 25  &     &                       &      &  \\
 c5221        & 0.1 &     &                  &         &     & 0.1 &  053832.458-690720.71 &   31,-22   & 23  &     &                       &      &  \\
 c5204        & 0.2 & 0.0 &                  & 8968459 &     & 0.1 &  053832.322-690314.89 &   14,-9    & 22  &     &                       &      &  \\
 c5122        & 0.1 & 0.3 &  686320819649024 &         &     &     &                       &            &     &     &                       &      &  \\
 cc3866       & 0.1 &     &                  &         &     & 0.3 &  053831.300-690722.45 &   34,-14   & 24  &     &                       &      &  \\
 pass52\_9    & 0.3 & 0.5 &                  & 9706008 & 18  &     &                       &            &     &     &                       &      &  \\
 c4979        & 0.1 &     &                  &         &     & 0.3 &  053829.768-690832.09 &   23,-14   & 24  &     &                       &      &  \\
 cc3671       & 0.2 &     &                  &         &     & 0.4 &  053828.462-690323.23 &   16,6     & 23  &     &                       &      &  \\
 c4784        & 0.1 & 0.2 &                  & 9777692 & 19  &     &                       &            &     &     &                       &      &  \\
 c4732        & 0.1 &     &                  &         &     & 0.2 &  053826.151-690306.44 &   11,22    & 26  &     &                       &      &  \\
 p1\_574      & 0.1 & 0.2 &                  & 9707046 & 18  &     &                       &            &     & 0.4 &   J053826.21-690012.9 & 16   &  \\
 p1\_567      & 0.1 & 0.1 &                  & 9774897 & 18  &     &                       &            &     &     &                       &      &  \\
 c4659        & 0.4 &     &                  &         &     &     &                       &            &     & 0.3 &   J053824.83-691704.3 & 16   &  \\
 c4620        & 0.2 & 0.4 &                  & 9769372 & 20  &     &                       &            &     &     &                       &      &  \\
 c4565        & 0.2 & 0.1 &                  & 9777952 & 20  &     &                       &            &     &     &                       &      &  \\
 cc3334       & 0.4 &     &                  &         &     & 0.9 &  053823.229-690119.32 &   -18,19   & 21  &     &                       &      &  \\
 c4555        & 0.1 &     &                  &         &     & 0.2 &  053823.034-690627.24 &   40,28    & 23  &     &                       &      &  \\
 cc3246       & 0.1 &     &                  &         &     & 0.4 &  053821.868-690415.16 &   29,41    & 21  &     &                       &      &  \\
 c4405        & 0.4 & 0.7 &  783490104306304 & 8855976 & 10  &     &                       &            &     & 0.9 &   J053821.25-685034.0 & 10   &  \\
 c4273        & 0.0 & 0.2 &                  & 9772852 & 20  &     &                       &            &     &     &                       &      &  \\
 cc2951       & 0.2 &     &                  &         &     & 0.6 &  053817.899-690756.49 &   29,46    & 25  &     &                       &      &  \\
 p1\_492      & 0.0 & 0.1 &                  & 9773515 & 18  &     &                       &            &     &     &                       &      &  \\
 c4107        & 0.2 &     &                  &         &     &     &                       &            &     & 0.5 &   J053816.23-692331.6 &  8   &  \\
 cc2768       & 0.2 &     &                  &         &     & 0.4 &  053815.445-690656.48 &   35,58    & 24  &     &                       &      &  \\
 p1\_488      & 0.5 & 0.3 &                  & 8904680 & 18  &     &                       &            &     & 0.3 &   J053814.99-685608.6 & 16   &  \\
 c3916        & 0.2 & 0.3 &  686698750750848 & 8976411 &     & 0.3 &  053810.121-690224.70 &   14,80    & 19  &     &                       &      &  \\
 p1\_464      & 0.2 & 0.3 &  688863422482304 & 8912592 & 16  &     &                       &            &     & 0.2 &   J053809.91-685657.7 & 15   &  \\
 c3887        & 0.2 & 0.3 &  686737399181568 &         &     &     &                       &            &     & 0.1 &   J053809.21-690121.0 & 16   &  \\
 c3847        & 0.3 &     &                  &         &     &     &                       &            &     & 0.4 &   J053808.36-690202.0 & 16   &  \\
 c3821        & 0.1 & 0.2 &                  & 9012120 & 18  &     &                       &            &     &     &                       &      &  \\
 c3801        & 0.2 &     &                  &         &     & 0.3 &  053807.411-690633.14 &   34,85    & 26  &     &                       &      &  \\
 c3775        & 0.2 &     &                  &         &     & 0.6 &  053806.273-691310.00 &   -37,46   & 24  & 0.8 &   J053806.27-691310.1 & 15   &  \\
 c3766        & 0.2 & 0.2 &  679968549406848 & 9021508 & 13  & 0.2 &  053805.644-690909.77 &   13,70    & 19  & 0.3 &   J053805.61-690909.6 & 11   &  YSO (2MASS6X J05380564-6909098)\\
 p1\_450      & 0.0 & 0.1 &                  & 9708672 & 19  & 0.1 &  053802.741-690259.15 &   24,105   & 22  & 0.1 &   J053802.73-690258.9 & 16   &  \\
 cc1809       & 0.2 &     &                  &         &     & 0.2 &  053801.499-690623.84 &   27,95    & 21  &     &                       &      &  \\
 p1\_445      & 0.1 & 0.3 &                  & 9779435 & 18  &     &                       &            &     &     &                       &      &  \\
 c3614        & 0.3 &     &                  &         &     &     &                       &            &     & 0.3 &   J053800.32-690031.0 & 16   &  \\
 cc1686       & 0.3 &     &                  &         &     & 0.8 &  053759.565-690437.66 &   26,107   & 22  &     &                       &      &  \\
 c3526        & 0.2 & 0.6 &                  & 8872736 & 17  &     &                       &            &     & 0.7 &   J053757.84-685238.2 & 16   &  \\
 p1\_410      & 0.1 & 0.3 &                  & 9710167 & 16  & 0.2 &  053754.561-690516.57 &   23,107   & 26  &     &                       &      &  \\
 p1\_406      & 0.1 & 0.1 &                  & 9771021 & 20  &     &                       &            &     & 0.0 &   J053754.32-690222.1 & 17   &  \\
 p1\_394      & 0.1 &     &                  &         &     &     &                       &            &     & 0.5 &   J053753.26-690302.1 & 16   &  \\
 c3078        & 0.2 &     &                  &         &     & 0.5 &  053751.827-690759.48 &   11,92    & 24  &     &                       &      &  \\
 c2505        & 0.6 & 0.5 &  700786243245056 & 8895601 & 17  &     &                       &            &     &     &                       &      &  \\
 c2202        & 0.5 & 0.5 &  701198560089088 & 8877930 & 17  &     &                       &            &     & 0.5 &   J053745.77-685311.3 & 15   & AGN (MQS J053745.77-685311.4) \\
 c2239        & 0.2 &     &                  &         &     &     &                       &            &     & 0.4 &   J053745.77-690435.4 & 17   &  \\
 c1348        & 0.5 & 0.6 &                  & 9705614 & 16  &     &                       &            &     & 0.5 &   J053738.09-685753.1 & 15   &  \\
 c1286        & 0.4 & 0.4 &                  & 9781489 & 20  &     &                       &            &     &     &                       &      &  \\
 p1\_22       & 0.1 & 0.2 &                  & 9771220 & 18  &     &                       &            &     &     &                       &      &  \\
 cc226        & 0.3 &     &                  &         &     &     &                       &            &     & 0.5 &   J053733.91-690307.0 & 17   &  \\
 c1205        & 0.1 &     &                  &         &     &     &                       &            &     & 0.6 &   J053732.37-690507.6 & 17   &  \\
 p1\_14       & 0.1 & 0.1 &                  & 9772860 & 20  &     &                       &            &     &     &                       &      &  \\
 c1167        & 0.2 & 0.5 &  692024485433088 & 8982580 & 16  &     &                       &            &     & 0.2 &   J053729.61-690451.8 & 16   &  \\
 c1154        & 0.4 & 0.3 &                  & 9771759 & 19  &     &                       &            &     &     &                       &      &  \\
 p1\_12       & 0.2 & 0.3 &                  & 9779274 & 19  & 0.2 &  053727.563-691218.70 &   12,58    & 24  &     &                       &      &  \\
 c1155        & 0.5 & 1.1 &                  & 9107666 & 16  &     &                       &            &     & 0.9 &   J053726.92-691805.1 & 16   &  \\
 c1136        & 0.5 & 0.6 &                  & 9781022 & 19  &     &                       &            &     &     &                       &      &  \\
 p1\_11       & 0.2 & 0.2 &                  & 9711726 & 17  & 0.2 &  053725.617-690738.37 &   -12,29   & 25  & 0.4 &   J053725.55-690738.2 & 16   &  \\
 c1087        & 0.4 & 0.2 &                  & 9771060 & 18  &     &                       &            &     & 0.4 &   J053723.63-690223.7 & 16   &  \\
 c1042        & 0.3 &     &                  &         &     & 0.3 &  053721.382-690621.28 &   -13,11   & 26  & 0.6 &   J053721.45-690621.4 & 17   &  \\
 c965         & 0.3 & 0.3 &                  & 8967015 & 18  &     &                       &            &     &     &                       &      &  \\
 c963         & 0.2 & 0.2 &                  & 9059422 & 17  &     &                       &            &     & 0.5 &   J053715.23-691316.1 & 16   &  \\
 c979         & 1.1 & 1.9 &  663849561921024 & 9131446 &     &     &                       &            &     & 1.5 &   J053714.70-692021.0 & 17   &  \\
 c919         & 0.3 & 0.2 &  690001595436160 & 9033573 & 15  & 0.2 &  053710.840-691025.19 &   49,51    & 18  & 0.4 &   J053710.87-691025.1 & 14   &  \\
 c865         & 0.3 &     &                  &         &     & 0.4 &  053707.530-691243.60 &   144,135  & 23  &     &                       &      &  \\
 c809         & 0.2 & 0.4 &                  & 9772081 & 20  &     &                       &            &     &     &                       &      &  \\
 p1\_5        & 0.3 & 0.4 &  690070295111040 & 9025732 & 18  &     &                       &            &     & 0.5 &   J053703.80-690942.6 & 17   &  \\
 cc60         & 1.0 &     &                  &         &     & 1.6 &  053659.745-690813.01 &   38,-16   & 21  &     &                       &      &  \\
 c749         & 0.4 & 0.7 &  693433288582784 & 8962789 & 16  &     &                       &            &     & 0.6 &   J053658.57-690234.2 & 16   &  \\
 pass53\_1    & 0.2 & 0.3 &  666323458738560 & 9061522 & 15  & 0.3 &  053657.042-691328.57 &   309,290  & 21  & 0.1 &   J053657.12-691328.2 & 14   &  \\
 c718         & 0.4 & 0.4 &                  & 8954856 & 17  &     &                       &            &     & 0.4 &   J053654.58-690138.0 & 16   &  \\
 c681         & 0.4 & 0.7 &                  & 9091631 & 17  &     &                       &            &     &     &                       &      &  \\
 c373         & 0.9 & 0.8 &  702989558190336 & 8894623 & 14  &     &                       &            &     & 0.8 &   J053612.44-685455.9 & 14   &  \\
 c298         & 0.8 & 1.4 &                  & 8962330 & 19  &     &                       &            &     &     &                       &      &  \\
 c73          & 0.2 & 0.5 &                  & 9090770 & 15  &     &                       &            &     &     &                       &      &  SNR 1987A\\
 c1           & 1.8 & 2.2 &                  & 8985162 & 20  &     &                       &            &     &     &                       &      &  
\enddata
\tablecomments{

}
\tablenotetext{a}{
Column ``ID'' is the published label for a detection in the HTTP catalog.  Column ``Correction'' reports the shift we applied to the published position.
}
\tablenotetext{b}{
Separation between ACIS source and Adopted Coordinates.
}
\tablenotetext{c}{
Identifiers reported by SIMBAD.
}
\tablenotetext{d}{Using our judgement, we assert two associations that were not found by automated methods:
Pulsar PSR~J0537-6910 == T-Rex 053747.40-691020.2 (p1\_255);
the low-mass star HD~269921 == T-ReX  053834.66-685306.1 (pass52\_4).}
%
%\vspace*{3em}
\end{deluxetable}
\end{longrotatetable}

